Semantic 3D Reconstruction with Finite Element Bases

We propose a novel framework for the discretisation of multi-label problems on arbitrary, continuous domains. Our work bridges the gap between general FEM discretisations, and labeling problems that arise in a variety of computer vision tasks, including for instance those derived from the generalised Potts model. Starting from the popular formulation of labeling as a convex relaxation by functional lifting, we show that FEM discretisation is valid for the most general case, where the regulariser is anisotropic and non-metric. While our findings are generic and applicable to different vision problems, we demonstrate their practical implementation in the context of semantic 3D reconstruction, where such regularisers have proved particularly beneficial. The proposed FEM approach leads to a smaller memory footprint as well as faster computation, and it constitutes a very simple way to enable variable, adaptive resolution within the same model.

==> justPaperArxiv/tabulars/verification.tex <==
\begin{table}
\centering
\setlength\tabcolsep{5pt}
\begin{minipage}{0.45\textwidth}
%\begin{minipage}{0.48\textwidth}
\centering
%\tablewidth=\textwidth
%
\begin{tabular}{l|c|c|c}
{\bf ov.\ acc.\ [\%]} & Tetra & Octree & MBoost \\ \hline
Scene 1 & 84.0 & 83.9 & 82.5 \\
Scene 2 & ... & ... & ... \\
\end{tabular}
%
% OLD VERSION
%
%\begin{tabularx}{\columnwidth}{l|X|c|c|c}
%Data set & Error measure & Tetra & Octree & MB \\\hhline{=|=|=|=|=}
%\multirow{2}{*}{Scene 1} 
% & Ov.\ acc. [\%] & 84.0 & 83.9 & 82.5 \\
% & Average acc. [\%] & 81.1 & 80.6 & 81.4 \\
% 
%\hline
%\multirow{2}{*}{Scene 2} 
% & Ov.\ acc. [\%]& ... & ... & ... \\
% & Average acc. [\%]& ... & ... & ... \\
%\end{tabularx}
%
%\vspace{-0.2cm}
\caption{Quantitative comparison with octree model and MultiBoost input data.}
\label{tab:verified} 
\end{minipage}%
\hfill
\begin{minipage}{0.48\textwidth}
\centering
%
\begin{tabular}{l|c|c}
 & memory[GB] & runtime[sec] \\\hline
basic & ... & ... \\
adaptive & ... & ...    
\end{tabular}
%
% OLD VERSION
%
%\begin{tabularx}{\columnwidth}{X|c|c}
%Version & Memory[GB] & Runtime[sec] \\\hhline{=|=|=} 
%Non-Adaptive & ... & ... \\ \hline
%Adaptive & ... & ...    
%\end{tabularx}
%\vspace{-0.2cm}
 \caption{Memory footprint and run-time of basic and adaptive FEM methods for large-scale city reconstruction (\emph{cf.} Fig.\ref{fig:3d_reconstruction}).} 
 \label{tab:adaptive_gains} 
\end{minipage}
\end{table}


==> justPaperArxiv/tabulars/verificationX.tex <==
\begin{table}[h]

  \centering
  \setlength\tabcolsep{5pt}
  %\small
  \begin{tabular}{ l|c|c|c|c|c }

Data set & Error measure & Tetra P1 & Tetra RT & Octree & MB \\ \hline
\multirow{2}{*}{Scene 1} 
 & Overall acc. [\%] & 84.0 & 81.9 & 83.9 & 82.5 \\
 & Average acc. [\%] & 81.1 & 79.1 & 80.6 & 81.4 \\

  \end{tabular}
\vspace{2mm}
\caption{Quantitative comparison of our two proposed FEM methods with octree model \cite{BlahaVRWPS16} and MultiBoost input data \cite{benbouzid_jml12}.}
\label{tab:verifiedX}
\vspace{-0.45cm}
\end{table}


==> justPaperArxiv/tex/conclusion_-_Copy.tex <==

%
Our basic idea is generic and not limited to semantic 3D
reconstruction or the specific class of regularizers.
We would like to explore other applications where it may be useful
to abandon grid discretizations and move to a decomposition into simplices.

\textcolor{Konrad}{This is BMVC -- use British English, respectively
  British spellchecker. regulariSe, optimiSe, discretiSe, neighbOUr,
  colOUr, \etc}


==> justPaperArxiv/tex/methods_endlines.tex <==
%
The multi-labeling
problem \cite{ChambolleCP12,Strekalovskiy11,Lellmann11,ZachHP14} in
the domain $\Omega\subset \mathbb{R}^d$ is defined by finding $m$
labeling functions $x^i:\Omega \rightarrow \{0,1\}, i=1\ldots m$ as
the solution of:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:multiLabelProblem}
%\begin{split}
\inf_{x^i} \sum_{i=1}^m \int_\Omega \rho^i(z) x^i(z) \dz + J(x^i),
\quad\textrm{s.\ t. } \sum_{i=1}^{m} x^i(z)=1 \;\forall z\in\Omega,
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
where $\rho$ models the data term for a specific label at location
$z\in\Omega$ and $J$ denotes a convex regularisation functional that enforces
the spatial consistency of the labels.
%
\textcolor{Christoph}
{
One prominent example is to chose $J:= \norm{\cdot}{_2}$, known as Total Variation,
which penalises the perimeter of the individual regions
\cite{ChambolleCP12,NieuwenhuisTC13}.
%
Note that in the the two-label case (Potts model), this relaxation is exact
after thresholding with any threshold from the open unit
interval \cite{ChambolleCP12}.
%-> generalised Potts model -- should be clear now .. it is stupid to refer to the abstract here .. ?
}
%
Although we are ultimately interested in non-metric regularisation, we
start with the continuous, anisotropic model \cite{Strekalovskiy11},
and postpone the extension to the non-metric case to Sec.~\ref{subsec:nonmetric}.
%and postpone the extension to the non-metric case,
%and a discussion of its implications to Sec.~\ref{subsec:nonmetric}.

\vspace{-0.9em}
\subsection{Convex Relaxation}
\vspace{-0.3em}
%
The continuous model allows for an anisotropic regulariser in $J$:
label transitions can be penalised on the area of the shared surface,
as well as on the surface normal direction.
%
This is achieved with problem-specific 1-homogeneous functions that
emerge from convex sets, so called Wulff-shapes.
%instead of unit balls.
%As mentioned, we choose for $J$ the anisotropic model of \cite{Strekalovskiy11}
%and extend it later to the non-metric case, after discretisation.
%
A relaxation of $x^i(z)\in\{ 0,1\}$ to $x^i(z)\in[0,1]$ then leads to a convex
energy, which can be written as the following saddle point problem, with primal functions $x$ and dual functions $\lambda$:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:saddle}
%\begin{split}
%&
\min_{x^i} \max_{\lambda^i} \sum_i\!\!\! \int_\Omega\!\!\!\! \rho^i\!(z) x^i(z) \!\!+\!\! \langle x^i(z), \div \lambda^i(z) \rangle \dz,
%\\
%&
\;\;
\textrm{s.t. } \lambda^i(z)\!-\!\lambda^j(z) \in W^{ij}\!\!
, %\textrm{ and }
\sum_{i=1}^{m} \!x^i(z)\!\!=\!\!1 , %\raisetag{3.5\baselineskip} %\notag
x^i(z)\!\geq\!0 .
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
%where the labeling function $x^i:\Omega \rightarrow \mathbb{R}$
The constraints have to be fulfilled for all $z\in\Omega$.
In addition to the primal variables $x^i$, we have introduced the dual
vector-field $\lambda^i:\mathbb{R}^d\rightarrow \mathbb{R}^d$, whose pairwise
differences are constrained to lie in the convex sets (Wulff-shapes) $W^{ij}$.
%
By letting these shapes take an anisotropic form, one can then encode
scene structure, \eg \cite{Strekalovskiy11,HaneZCAP13}.  For our
problem we demand Neumann conditions at the boundary of $\Omega$, \ie
$\langle \lambda^i,\nu \rangle =0,\forall z\in\partial\Omega$,
because the scene will continue beyond our domain ($\nu$ is the normal
of the domain boundary $\partial \Omega$).
%
%\todo{Test functions H1 div conforming spaces weak form .. NO}

\vspace{-0.7em}
\subsection{Finite Element Spaces}
\vspace{-0.3em}
%
Here, we can only informally introduce the basic idea of FEM and
explain its suitability for problems of the form
\eqref{eq:saddle}. We refer to textbooks
\cite{Larson2013FEM,Brezzi1991,Duran2008} for a deeper and
formal treatment.
%
%In a nutshell, FEM consists in searching a solution of a variational problem

One way to solve ~\eqref{eq:saddle} is to approximate it at
a finite number of regular grid points, using finite
differences.
%
%The fundamental difference to FEM is that in the latter case we search
%A fundamental difference to FEM is that here we search
%A fundamental difference to FEM is that here we search
\textcolor{Christoph}{FEM instead searches} %shorter !
for a solution in a finite-dimensional vector space;
this \emph{trial} space is a subspace of the space in which the exact
solution is defined.
%
To that end, one chooses a suitable basis for the \emph{trial} space,
with basis functions of finite support, as well as an
appropriate \emph{test} function space.
%These must not necessarily coincide \cite{Duran2008}. % petrov galerkin
%
FEM methods then find approximate solutions to variational problems by
identifying the element from the \emph{trial} space that is orthogonal to all
functions of the \emph{test} function space.
% orthogonal means wrt inner product, given by integral (function space inner product)
For our saddle-point problem, we can instead identify the \emph{trial} space with
our primal function space and the \emph{test} space with its dual counterpart.
% then eg. max -> neccessary condition is derivative == 0 ; which is
%
Now, we can apply the same principles, and after discretisation our
solution corresponds to the continuous solution defined
by the respective basis.
%which we will in the following. %derive from here.
%
\begin{comment}
% SHORTEN !!
%Note, that consider sequences of subspaces converging to the original space.
We do not perform any convergence analysis, which would be to
consider sequences of subspaces converging to the original space.
This topic goes beyond the scope of this work.
%
The interested reader is referred to \cite{Bartels12}
for a study \wrt Total Variation.
%
Further, we are only dealing with the convex relaxation \eqref{eq:saddle}
of the original problem \eqref{eq:multiLabelProblem}.
%
\end{comment}
% shorter !
%Because we are dealing with the convex relaxation \eqref{eq:saddle}
%of the original problem \eqref{eq:multiLabelProblem}, we are not
%analyzing the convergence properties of our method.
%
%
%but also due to the complexity
%of an analysis of convergence we
%refer the interested reader to \cite{Bartels12} for a
%study concerning Total Variation.
%
% beyond the scope of this work.
%
%We consider An analysis of the convergence of goes beyond the scope of this work.
As \eqref{eq:saddle} is already a relaxation of the original
problem \eqref{eq:multiLabelProblem}, we do not present an analysis of
convergence at this point.
%
Instead, the reader is referred to \cite{Bartels12} for an
introduction to this somewhat involved topic.
%for a study concerning Total Variation.
%

In order to choose a space with good approximation properties and
suitable basis functions, we tesselate our domain into simplices.
%To define our subspace we assume a tesselation of our domain into simplices.
%To define our subspace we tesselate of our domain into simplices.
% or in next senstence more form.. to define our subspace we let
%
More formally, we define $M\!=\!\{F,V,S\}$ to be a simplex mesh with
vertices $v\!\in\! V, v\!\in\!\mathbb{R}^d$, faces $f\!\in\! F$ defined by $d$,
%vertices
and simplices $s\!\in\! S$, defined by $d\!+\!1$ vertices that
partition $\Omega$: $\cup_k s_k=\Omega, s_l\cap s_k\!=\!f_{l,k}\!\in\! F$
-- \ie two adjacent simplices share only a single face.
%
%In this work we let
In this work, for a specific set of vertices $V$, we select M to be
the corresponding Delaunay tetrahedralisation of $\Omega$
%
and only consider explicit bases. In particular, we
focus on the Lagrangian (P1) basis, which we use in the following to
derive our framework; and on the Raviart-Thomas (RT) basis.
Details for the latter are given in the supplementary material.
%, for lack of space.
%
The main difference between them is that P1 leads to piecewise linear
solutions, which must be thresholded, while RT leads to a constant
labeling function per simplex, similar to discrete MAP solutions on CRFs.
%
We note that constant labeling can lead to artefacts, such that the
adaptiveness of the FEM model becomes even more important.

%Both derivations share similar principles:
The idea of both derivations is similar:
\emph{(i)} select a basis for our primal (P1) or dual (RT) variable set,
\emph{(ii)} find a suitable form via the divergence theorem and Fenchel duality,
\emph{(iii)} extend to the non-metric case, following a principle we term ''label mass preservation''.
%Apply To fulfill our constraint set
%a complete
%derivation similar
%
\vspace{-0.7em}
\subsection{Lagrange Elements}
\vspace{-0.3em}
%
%The Lagrange $\textrm{P}^k(M)$ basis functions describe a
%div-conforming \textcolor{red}{the expression ``div-conforming'' is a
%bit too abstract to understand for most readers} polynomial basis of
%order $k\!+\!1$ on our simplex mesh $M$.
%
The Lagrange $\textrm{P}^k(M)$ basis functions describe a
\emph{conforming} polynomial basis of
order $k\!+\!1$ on our simplex mesh $M$, \ie its elements
belong to the Hilbert space of differentiable function with
finite Lebesgue measure on the domain $\Omega$:
$\textrm{P}^k(M)\subset H^1(\Omega):= \{ p\in L^2(\Omega),\nabla p\in(L^2(\Omega)^d) \}$.
%
%here, on a
%simplex mesh $M=\{F,V,S\}$ with vertices $v\in V, v\in\mathbb{R}^d$
%faces $f\in F$ defined by $d$ vertices and
%simplices $s\in S$, defined by $d+1$ vertices, that partition $\Omega$:
%$\cup_k s_k=\Omega, s_l\cap s_k=f_{s,k}\in F$.
%Here, two simplices share a single face.
%
We are interested in the Lagrange basis of first order, $\textrm{P}^1(M)$:
%
\vspace{-.125cm}
\begin{align}
P^1(M) \!\!:=\! \{\! p\!:\Omega\!\rightarrow\! \mathbb{R} | p \!\in\! C(\Omega), \,p(x)\!:=\!\sum_{s\in S} c_s\trans x + d_s, c_s\!\in\!\mathbb{R}^d, d_s\!\in \!\mathbb{R},
\textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else}\} .
\vspace{-.125cm}
\end{align}
%
We construct our linear basis with functions that are defined
for each vertex $v$ of a simplex $s$ and can be described in
local form with barycentric coordinates:
\vspace{-0.125cm}
\begin{equation}\label{eq:bariz}
p^{1}_{s,v}(x)   := \alpha_v\; \textrm{with } x=\sum_{v\in s} \alpha_v v, \; \sum_{v\in s} \alpha_v=1, \; \alpha_v\geq0 \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else}.
\vspace{-0.125cm}
\end{equation}
%
In each simplex, one can define a scalar field $\phi_s(x)\in\mathbb{R}$ and
compute a gradient in this basis that will be constant
per simplex $s$ (\textit{cf.} Fig. \ref{fig:lagrange_elements}):
\vspace{-0.125cm}
\begin{equation}\label{eq:gradient}
\phi_s(x) := \sum_{v\in s} \phi_v p^{1}_{s,v} \; \textrm{ and } \nabla \phi_s = \sum_{v\in s} \phi_v J_{v},
\vspace{-0.125cm}
\end{equation}
%
with coefficients $\phi_v\in \mathbb{R}$. $J_{v}\in\mathbb{R}^d$
denotes a vector that is normal to the face $f_v$ opposite node $v$,
has length $\frac{|f_v|}{|s|d}$, and points towards the simplex centre.
%
$|f_v|$ denotes the area of the face $f_v$,
and $|s|$
%$\frac{1}{d\!\cdot\!(d+1)}|s|$
the volume of the simplex $s$
(\cf \Fig\ref{fig:lagrange_elements} and supplementary material).
%

\begin{comment}
\textcolor{Christoph}{save space put in supp.:}
It is easy to see that the gradient of $\phi_t$ in (\ref{eq:gradient})
 fulfills $\langle v_l-v_k; \nabla \phi_t \rangle =
f_l-f_k$.
\Ie integration along the edge leads to the respective change
in $\phi_t$.  After collecting a sufficient number linear equations of this
form, one can directly solve the linear system.
By noting that $J_{v}$ is orthogonal to all edges that do not involve
vertex $v$ we arrive at \eqref{eq:gradient}.
\end{comment}
%

\begin{figure}[tb]
\begin{center}
   %\vspace{-3mm}
   \includegraphics[width=0.85\linewidth]{figures/lagrange_elements_v2.png}
\end{center}
   %\vspace{-6.25mm}
   \vspace{-5mm} \caption{\textcolor{Audrey}{\textit{Left:} Illustration of P1 basis function shape. \textit{Middle:} Scalar field defined as a convex combination of basis coefficients. \textit{Right:} Gradient definition in a simplex (\ref{eq:gradient}).}}
\label{fig:lagrange_elements}
\vspace{-4mm}
\end{figure}

\vspace{-0.7em}
\subsection{Discretisation}
\label{subsec:discretisation}
\vspace{-0.3em}
%
To apply our Lagrange basis to \eqref{eq:saddle} we first
make use of the divergence theorem:
%
\vspace{-0.075cm}
\begin{equation}\label{eq:p1_div}
%\begin{split}
\int_\Omega \langle x^i(z), \div \lambda^i(z) \rangle \dz =
\;
\int_\Omega \langle \nabla x^i(z), \lambda^i(z) \rangle \dz -
\underbrace{\int_{\partial\Omega} \langle \nu(z), \lambda^i(z) \rangle \dz}_{=0} .
%\end{split}
\vspace{-0.25cm}
\end{equation}
%
The latter summand vanishes by our choice of $\lambda$.
%
Our approach for a discretisation in the Lagrange basis is to
choose the labeling function $x^i\in P^1(M)$.
%The respective dual (\emph{test}) space consists of constant
%vector-field per simplex and thus also our dual vector-field
%$\lambda^i_{|s}\in\mathbb{R}^d$ is constant.
This implies that our dual space consists of constant vector-fields
per simplex: $\lambda^i_{s}\in\mathbb{R}^d$.
%
To fulfill the constraint set in \eqref{eq:saddle} we have to verify
that, per simplex, the $\lambda^i_{s}$ lie in the respective Wulff-shape.
%
%Naturally, we receive $\lambda^i_{|s}$ constant per simplex,
% similar to the gradient \eqref{}.
%Further, we observe that the constraints in \eqref{eq:saddle} are
%trivial to verify, the $\lambda^i$ are constant per simplex $s$,
%thus it is sufficient to verify that each constant vector lies in the
%respective Wulff-shape.
The simplex constraints on the $x^i$ have to be modeled per vertex.
According to \eqref{eq:bariz}, the labeling functions are convex
combinations of their values at the vertices and thus stay within the
simplex.
%
%Within the simplices the labeling functions are convex combinations
%of their values at the vertices, and thus stay inside the convex shape.

We also have to convert the continuous data costs $\rho^i$ into a
cost per vertex $\rho^i_v$, which can be achieved by
convolving the continuous cost with the respective basis function:
$\rho^i_v := \int_\Omega \sum_{s\in\mathcal{N}(v)} \phi_{s}(x) \rho^i(x)\dx$.
In practice, the integral can be computed by sampling $\rho$.
% todo also in sec 4 -> can go, save space
%
%After applying \eqref{eq:p1_div}, the energy \eqref{eq:saddle}
%in the discrete setting becomes:
%
% save a line, move above eq.: actually the shitty format uses the line to increase white space..
Integrating the right hand side in \eqref{eq:p1_div} over the simplex
$s$ leads to a weighting with its volume $|s|$ and the
energy \eqref{eq:saddle} in the discrete setting becomes:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:pd1_discrete}
%\begin{split}
\min_{x^i}\max_{\lambda^i}
\sum_v \rho^i_v x_v^i \!+\! \sum_s |s| \langle \nabla x^i, \lambda_s^i \rangle \;\; \textrm{s.t. }
%\\
(\!\lambda_s^i-\lambda_s^j\!)\! \in\! W^{ij} \;\forall i\!<\!j,\; s\in S
, %\textrm{ and }
\sum_{i=1}^{m} \!x_v^i\!\!=\!\!1, \; x_v^i\!\geq\!0 \;\forall v\!\in\! V. %\raisetag{2.5\baselineskip}
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
% save a line, move above eq.:
%The weighting term $|s|$ arises from integrating the
%right hand side in \eqref{eq:p1_div} %cost of the regularizer
%over the simplex $s$.
%
%
%reflects that the cost induced by the
%regularizer has to be integrated over the simplex $s$.
%
%follows from the fact that one has to integrate over
%the volume of the simplex, similar to the suggested definition of
%$\rho^i_v$ given above.

\subsection{Non-metric extension}
\label{subsec:nonmetric}
%
To start with, we note that a non-metric model does not exist in the
continuous case \cite{maggi2012sets} and our extension works
only \emph{after} the discretisation into the FEM basis.  Please refer
to the supplementary material for an in-depth discussion.
%
\textcolor{Christoph}
{Note that our label set of semantic classes does not have a natural
order (in contrast to, \eg, stereo depth or denoised brightness); and
also the direction-dependent regulariser is unordered and does not
induce a metric cost.  }
%
%This leads to the situation that we cannot find an order of our
%label set which allows our regulariser to be metric,
%\ie $\forall i<j<k: |y^{ij}|_W + |y^{jk}|_W \geq |y^{ik}|_W$.
%
%However, it was shown, \eg\cite{ZachHP14}, that a regularizer in the form
%of \eqref{eq:tranform1} transforms any non-metric cost to the metric case
%The situation is depicted in \Fig\ref{fig:xxx}.
%
%
%It should be noted that, since our model is designed for the
%non-metric relaxation of \cite{ZachHP14},
%which does not posses a continuous counterpart
%convergence to the continuous solution cannot be shown.
%
%
To allow for non-metric regularisation we transform the constraint set
($\lambda^i-\lambda^j\in W^{ij}$), by introducing auxiliary
variables $z^{ij}$ and Lagrange multipliers $y^{ij}$, and use
Fenchel-Duality:
%
%We now simplify our constraint set ($\lambda^i-\lambda^j\in W^{ij}$),
%to transform our energy to utilise non-metric
%Wulff-shapes.
%
%To that end, we introduce auxilliary variables $z^{ij}$ and
%Lagrange multipliers $y^{ij}$ and exploit Fenchel-Duality:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:tranform1}
%\begin{split}
\max_{\lambda_s^{i},z_s^{ij}}\min_{y_s^{ij}}
\sum_{i<j}
\langle (\lambda_s^i-\lambda_s^j)-z^{ij}, y_s^{ij} \rangle - \delta_{W^{ij}}(z_s^{ij})
=
\max_{\lambda_s^{i}}\min_{y_s^{ij}}
\sum_{i<j}
- \langle (\lambda_s^i-\lambda_s^j), y_s^{ij} \rangle + || y_s^{ij} ||_{W^{ij}}.
%\end{split}
\vspace{-0.1cm}
\end{equation}
%\sum_v \rho^i_v x_v^i + |s| || y_s^{ij} ||_{W^{ij}}
The dual functions of the indicator functions for the convex
sets $W^{ij}$ are 1-homogeneous, of the form
$|| \cdot ||_{W^{ij}} \!:=\! \sup_{w\in W^{ij}} w\trans \cdot$.
%
%After rearranging terms and ignoring data term %, regularisers
%simplex constraints
%and also the weighting term $|s|$ for now,
%
\textcolor{Christoph}
{
%As explained, there is no order of our
%label set that allows to formulate our regulariser as a metric,
%
%Recall that we cannot order our labels such that
%our regulariser forms a metric on the label set,
Recall that our label costs are not metric:
$\forall i\!<\!j\!<\!k: |y^{ij}|_{W^{ij}} + |y^{jk}|_{W^{jk}} \geq |y^{ik}|_{W^{ik}}$,
does not hold.
%
It was shown \cite{ZachHP14} that a regulariser of the form
\eqref{eq:tranform1} transforms any non-metric cost to the metric case.
%In other words \eqref{eq:pd1_discrete} cannot handle non-metric regularisers.
Figure \ref{fig:non-metricness} shows an example.  Here, an
expensive transition between labels 0 and 2 will be replaced by
two cheaper transitions 0--1 and 1--2.
%with a detour via label 1.
To prevent this, we replace the $y^{ij}$ with direction dependent variables
$x^{ij}$: % and demand the transported label mass in $x^{ij}$ to be positive.
%
%by the transition via label 1
%cost by the non-metric
%expensive transition
%After rearranging
%To that end,
We rearrange \eqref{eq:tranform1}
}
and combine the first summand % in \eqref{eq:tranform1}
with the regulariser
from \eqref{eq:pd1_discrete} to arrive at the following equations
(for now ignoring $|s|$):
%
\vspace{-0.1cm}
\begin{equation*}
\sum_s \sum_i\langle \nabla x^i, \lambda_s^i \rangle
-  \sum_i \langle \lambda_s^i, \sum_{j\neq i} \left(y_s^{ij}[i<j]-y_s^{ji}[i>j] \right)\rangle, % + || y_s^{ij} ||_{W^{ij}},
\vspace{-0.1cm}
\end{equation*}
%
with $[\cdot]$ denoting Iverson brackets.
%
Let $x^{ij}:= [y^{ij}]_+$ and $x^{ji}:= [-y^{ji}]_+$,
where $[\cdot]_+:=\max(0,\cdot)$. Expanding the gradient
\eqref{eq:gradient} we get, per  simplex $s$,
%
\vspace{-0.1cm}
\begin{equation}
\sum_i \sum_{v\in s} \lambda^i_s x_v^i( [J_{v}]_+ - [-J_{v}]_+)
- \langle \lambda_s^i, \sum_{j:i\neq j} (x^{ij}-x^{ji}) \rangle,
\vspace{-0.14cm} % todo set to 0.44 and shorter .. but looks a bit off not totally though
\end{equation}
which we analyse further to achieve non-metric costs.
%
%To arrive at the discrete non-metric form,
It was observed in \cite{ZachHP14} that the $x^{ij}\in\mathbb{R}^d$
can be interpreted as encoding the ``label mass'' that transitions
from label $i$ to label $j$ in a specific direction.
%, encoded by the variables.
%
Positivity constraints (by definition) on the $x^{ij}$ avoid
the transport of negative label mass.
%
%
%\footnote{A ``positive'' direction for each component is arbitrarily,
%but consistently defined by the coordinate system.} %
%
%Further the gradient $\nabla x^i$ has to be explained
To anchor transport of mass on the actual mass of label $i$ present at
a vertex, we introduce the variables $x^{ii}$ for the mass that
remains at label $i$, and split the above constraints into two separate sets
with the help of additional dual variables $\theta$:
%
\vspace{-0.075cm}
\begin{equation}\label{eq:nonMetric}
%
\lambda^i_s (\sum_{v\in s} x_v^i [ J_{v}]_+ - \sum_j x_s^{ij}) +
\theta^i_s  (\sum_{v\in s} x_v^i [-J_{v}]_+ - \sum_j x_s^{ji}) +
\sum_{i,j} \delta_{\geq0}(x_s^{ij}).
\vspace{-0.075cm}
\end{equation}
%

\begin{figure}[t]
\begin{center}
   %\vspace{-1mm}
   \includegraphics[width=0.9\linewidth]{figures/non-metricness_v3.png}
\end{center}
   %\vspace{-6.25mm}
%   \vspace{-5mm} \caption{\textcolor{Christoph}{\textit{Left:} Without our non-metric extension,
%	optimization \wrt \eqref{eq:pd1_discrete} can lower transition costs between labels via an
%	intermediate label (here from 0 to 2 via label 1).
%	\textit{Right:} To prevent this, we use direction dependent transition variables $x^{ij}$.
%	}}
   \vspace{-5mm} \caption{\textcolor{Christoph}{\textit{Left:} Without
	our non-metric extension,
	optimisation \wrt \eqref{eq:pd1_discrete} can lower transition
	costs by inserting another label (here 1 between 0 and
	2).  \textit{Right:} A solution is to split the
	gradients of the indicator functions and use direction-dependent
	variables $x^{ij}$. %of the $x^i$ indicator fcts.
	}}
%
%   \vspace{-5mm} \caption{\textcolor{Audrey}{\textit{Left:} Synthetic scenes illustrate the effect of using (\ref{eq:pd1_discrete}) without the non-metric extension. For a transition \textit{building} to \textit{sky}, which should be highly penalized, the paid cost is in reality smaller, \textit{ie.} like if it was a proper transition \textit{building} to \textit{roof} and \textit{roof} to \textit{sky}. This results in the apparition of several unwanted transitions \textit{building} to \textit{sky} in our reconstruction. \textit{Right:} To circumvent it, the non-metric extension should be applied in order to obtain a correct assigned cost.}}
\label{fig:non-metricness}
\vspace{-3mm}
\end{figure}
%
\noindent
Note that this construction is only possible because our
elements (simplices) are of strictly positive volume,
in contrast to zero sets in $\Omega$ \wrt the Lebesgue measure.
%
%Further notice 1-homogeneous function
%which, again, are mandatory for the continuous case.
%and ensure that
%
Finally, we can write down our discrete energy in the Lagrange basis
defined on the simplex mesh $M$:
%
\vspace{-0.001cm}
\begin{equation}\label{eq:final}
\begin{split}
\min_{x^i, x^{ij}} \max_{\lambda^i,\theta^i}
%
&
\sum_{v\in V} \sum_i \rho^i_v x_v^i + \delta_{\Delta}(x_v^i) + \sum_{i<j} \sum_{s\in S} |s| || x_s^{ij}-x_s^{ji} ||_{W^{ij}} +
\\
&
\sum_s \sum_i \theta^i_s  (\sum_{v\in s} x_v^i [-J_{v}]_+ - \sum_j x_s^{ji})
%\\
+
%&
\sum_s \sum_i \lambda^i_s (\sum_{v\in s} x_v^i [ J_{v}]_+ - \sum_j x_s^{ij}) +
\sum_{i,j} \delta_{\geq0}(x_s^{ij}), \raisetag{3.5\baselineskip}
\end{split}
\vspace{-0.075cm}
\end{equation}
%
where we have moved the weighting with $|s|$ from the constraint set
to the regulariser, and denote by $\delta_{\Delta}(\cdot)$ the
indicator function of the unit simplex.
%




\vspace{-0.075cm}
\section{Semantic Reconstruction Model}\label{subsec:implementation}
%
A prime application scenario for our FEM multi-label energy model
\eqref{eq:final} is 3D semantic reconstruction.
%with scenes dominated by larger constant regions.
%where larger regions of constant labelings.
%
%
%We focus on an urban scenario and encode with
%As indicated by the respective function $(x^i=1)$, the voxels can take
%on a state (\ie a class) $i$ out of a predefined set
%$\mathcal{C}=\{0 \ldots M\}$.
%
In particular, we focus on an urban scenario and let our labeling
functions encode \emph{freespace} ($i=1$), \emph{building wall},
\emph{roof}, \emph{vegetation} or \emph{ground}.
Objects that are not explicitly modeled are collected in an
extra \emph{clutter} class.
%
We define the data cost $\rho$ at a 3D-point $x\in\Omega$ as in
\cite{HaneZCAP13}: project
$x$ into the camera views $c\in\mathcal{C}$, and retrieve the
corresponding depth $\hat{d}_c(x)$ and class likelihoods
$\sigma_c^i(x)$ from the image space.
%
The $\sigma^i$ are obtained from a MultiBoost classifier. For the depth we
look at the difference between the actual distance $d_c(x)$ to the
camera and the observed depth: $d(x,c):=d_c(x)-\hat{d}_c(x)$.
%
For the \emph{freespace} label we always set the cost to 0, for $i\neq
1$ we define:
%
%and also the distance of $x$
%to the camera $d_c(x)$ and use to define the distance between current and observed depth value.
%Then we can assign for $i\neq0$ \rho^i(x)
\vspace{-0.075cm}
\begin{equation}\label{eq:datacost}
\rho^i(x)\!:=\!\sum_{c\in\mathcal{C}}\! \sigma_c^i(x)[(k\!-1\!)\epsilon\leq d(x,c) \leq k\epsilon] +
\beta [|d(x,c)|\leq k\epsilon] \sign(d(x,c)).
%\rho^i(x)\!:=\!\sum_{c\in\mathcal{C}}\! \sigma_c^i(x)[(k\!-1\!)\epsilon\leq d_c(x)\!-\!\hat{d}_c(x)\leq k\epsilon] +
%\beta [|d_c(x)\!-\!\hat{d}_c(x)|\leq k\epsilon] \sign(d_c(x)\!-\!\hat{d}_c(x))
\vspace{-0.075cm}
\end{equation}
% todo nice figure in supplementary !! like integration thing !
%
% space ?
%The situation is depicted in \Fig\ref{fig:data}.  $\sigma^i$ denotes
%the negative log-likelihoods of observing class $i$ in the pixel.
%Details can be found in the supplementary material.
%
This model assumes independence of the per-pixel observations, and
exponentially distributed inlier noise in the depthmaps, bounded by a
parameter $k\epsilon$ (k=3 in practice). It is essentially a
continuous version of \cite{HaneZCAP13}, see that paper for details.
%
%Assuming independence of the per-pixel observations, %in different views and pixels,
%the final data costs per voxel can be accumulated over all rays. %simply
%
%
\textcolor{Christoph}{
The parameter $\epsilon$ sets a lower bound for the minimal height
of the simplices in the tesselation, and thus defines the target
resolution.
%bounds the minimal height of the simplices of our tesselation from below.
}
%
The discretisation of the data cost involves a convolution with the
respective basis functions, which can be approximated via sampling.
Please refer to the supplementary material for details.
%
% too long .. ?
%
\begin{comment}
%
Although we could employ importance sampling to define the data cost
$\rho^i_v$ and thus directly couple data term computation with the
construction of $M$, we resort to a much simpler strategy.
%
In \cite{HaneZCAP13} the data cost is evaluated on a regular grid, by
reprojecting grid vertices into the images, computing the data term and
adding the respective contribution to the grid location.
%
This corresponds to integrating the data cost within the respective
Voronoi-area of a vertex: the latter is proportional to the number of
regular samples falling within a Voronoi-cell, \ie have the respective
vertex as nearest neighbour.  Summing up the individual contribution
thus directly corresponds to integrating the data term within the
Voronoi region.
%
This procedure could easily be extended to importance sampling,
but it is not the computational bottleneck of the method, so we prefer
the simpler regular strategy.%
\end{comment}
%
%
The Wulff-shapes $W^{ij}$ in \eqref{eq:final} are given as the
Minkowski sum of the $L_2$-Ball,
$B^2_{\kappa^{ij}}:=\{x\in\mathbb{R}^d| \|x\|_2 \leq \kappa^{ij}\}$
and an anisotropic shape $\Psi^{ij}$:
$W^{ij}:= \Psi^{ij} \oplus B^2_{\kappa^{ij}}$.
%
In the isotropic part, $\kappa^{ij}$ contains the neighbourhood statistics
of the classes. The anisotropic part $\Psi^{ij}$ models the likelihood
of a transition between classes $i$ and $j$ in a certain direction.
\textcolor{Christoph}{
\Fig\ref{fig:wulff_shape} (a,b) shows an example.
}
%
\textcolor{Christoph}{
For our case we prefer flat, horizontal surfaces at the
following label transitions: \emph{ground-freespace}, \emph{ground-building},
\emph{building-roof}, \emph{ground-vegetation} and \emph{roof-freespace}.
%
A second prior prefers vertical boundaries for the transitions
\emph{building-freespace} and \emph{building-vegetation}.  More details on
the exact form can be found in \cite{HaneZCAP13}.  }
%
\begin{figure}[tb]
\begin{center}
   \vspace{-1mm}
   \includegraphics[width=0.95\linewidth]{figures/wulffshape_finitediff_split_v2.png}
\end{center}
   %\vspace{-6.25mm}
   \vspace{-5mm}
%	\caption{\textcolor{Audrey}{Not sure about this figure....}}
\caption[Optional caption for list of figures]{
\textcolor{Christoph}{
 \emph{(a):} Wulff-shape (\emph{red}) with isolines.
 \emph{(b):} Minkowski sum of two Wulff-shapes.
 \emph{(c):} Simplices are split after inserting new vertices (blue) close to the surface (green).
	\emph{Right:} Initialisation of vertices after refinement. % via barycentric coordinates.
\emph{(d):} Finite differences on a regular grid
  (\cite{HaneZCAP13}) only cover constraints in \emph{green} areas,
	the P1 basis covers all of the domain $\Omega$.
	}
}
\label{fig:wulff_shape}
\vspace{-3.5mm}
\end{figure}

The energy \eqref{eq:final} is already in primal-dual form, such that
we can apply the minimisation scheme of \cite{chambolle11}, with
pre-conditioning \cite{Pock11}.
%
That numerical scheme requires us to project onto shapes that are
Minkowski sums of convex sets.  In our case, the sets are simple and
the projection onto each shape can be performed in closed form.
%
We employ a Dykstra-like projection scheme \cite{Dykstra}, which
avoids storing additional variables and proves remarkably efficient,
see supplementary material.
%
We also project the labeling functions $x^i$ directly onto the unit
simplex \cite{WangC13a}.
%
In order to extract the transition surface, we employ a variant of marching
tetrahedra (triangles) \cite{treece1999mtet}, using the isolevel at $0.5$
for each label.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Comparison to Voxel Based Tesselation}

%\mypargraph{Remarks. }
% $x^i_{\hat{v}}:=\sum_{v\in s}  \alpha_v(\hat{v} )x^i_{v}$
%

%
% Other VERSION
%
%\begin{figure}[ht]
%\centering
%\subfigure[]{
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%    \label{fig:grid}
%}
%\hspace{0.4cm}
%\subfigure[]{
%\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%    \label{fig:refine}
%}
%
%\caption[Optional caption for list of figures]{(a) \emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%  \emph{Right:} Gradient definition in a simplex (\eqref{eq:gradient}).
% (b)\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface (green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%}
%\label{fig:subfigureExample}
%\end{figure}


%\begin{figure}[tb]
%\begin{minipage}{.575\textwidth}
%  \centering
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%	\vspace{-0.2cm}
%  \caption{\emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%%\emph{Right:} Gradient definition in a simplex \eqref{eq:gradient}.
%	}\label{fig:grid}
%\end{minipage}
%%
%\hspace{0.175cm}
%\begin{minipage}{.4\textwidth}
%  \centering
%	\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%		\vspace{-0.2cm}
%  \caption
%	{\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface (green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%	}\label{fig:refine}
%	%
%\end{minipage}
%\vspace{-4mm}
%\end{figure}



%\begin{figure}[tb]
%%\centering
%\begin{minipage}{.575\textwidth}
%  \centering
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%%	\vspace{-0.4cm}
%  \caption{\emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%\emph{Right:} Gradient definition in a simplex (\eqref{eq:gradient}).
%	}\label{fig:grid}
%\end{minipage}
%%
%\hspace{0.175cm}
%\begin{minipage}{.4\textwidth}
%  \centering
%	\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%		%\vspace{-0.4cm}
%  \caption
%	{\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface %(green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%	}\label{fig:refine}
%	%
%\end{minipage}
%\vspace{-5mm}
%\end{figure}


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[tb]
\centering
\includegraphics[width=0.175\columnwidth,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
\includegraphics[width=0.175\columnwidth,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual.pdf}
\includegraphics[width=0.15\columnwidth]{./figures/subdiv_Grad.pdf}
\hspace{0.3cm}
\includegraphics[width=0.375\columnwidth,trim={5cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%
\vspace{-0.1cm}
\caption{%Illustration of the
.
}\label{fig:grid}
\vspace{-0.3cm}
\end{figure}
\end{comment}
%
We conclude with two interesting remarks.
%
First, note that a tesselation with a regular grid \cite{HaneZCAP13} can be
seen as a simplified version of our discretisation in the $P^1$ Lagrange basis.
% consider the special case of a regular grid
%Consider a vertex set aligned on a grid, then we can a special case of
In \Fig \ref{fig:wulff_shape}(d) %\ref{fig:grid},
we consider the 2D case of the regular grid
%interpretation
used in \cite{HaneZCAP13}. Here, variables are defined at voxel level.
%
In its dual graph, the vertex set consists of the corners of the primal
grid cubes, leading to shifted indicator variables.  %are thus shifted;
Per vertex the data term is mainly influenced from the cost in its Voronoi area.
%
%and the dual cells correspond to the Voronoi cells of the
%dual vertex set.
%
Similarly, \cite{HaneZCAP13} evaluates the data cost at grid centers,
approximately corresponding to integration within the
respective Voronoi-area of grid cell. %a dual vertex.
%
Furthermore, taking finite differences in this regular case
corresponds to verifying constraints for %computing the gradient and
only one of the two triangles (\Fig\ref{fig:wulff_shape}(d)). %(\Fig \ref{fig:grid}).
The supplementary material includes a more formal analysis.
%
\begin{comment}
In the following we will show that a tesselation on a regular grid
\cite{HaneZCAP13} is a special case of our discretisation in the $P^1$ Lagrange
basis.
%
To that end, we consider the dual graph of a regular grid, \ie a grid where the
vertex set consists of corners of the primal grid cubes, and dual cells
correspond to voronoi cells \wrt new set of dual vertices.
%
For our regular grid the dual mesh simply becomes a shifted regular
grid \ref{fig:wulff_shape}(c). %\ref{fig:dual}.
%
\end{comment}

Second, our formulation is adaptive, in the sense
of \cite{BlahaVRWPS16}: Hierarchical refinement of the tesselation can
only decrease our energy. Hence, our scheme is applicable when refining
the model on-the-fly.
%
We again must defer a formal proof to the supplementary material and
give an intuitive, visual explanation in \Fig\ref{fig:wulff_shape}(c). % \Fig\ref{fig:refine}.
%
%Assume that we found an optimal solution $(x^*, \lambda^*, \theta^*)$
\textcolor{Christoph}{Assume that  $(x^*, \lambda^*, \theta^*)$ is an optimal solution}
for a certain triplet $M=\{F,V,S\}$.  Then a refined tesselation
$\hat{M}=\{\hat{F},\hat{V},\hat{S}\}$ can be found by introducing
additional vertices, \ie $V\subset\hat{V}$ (ideally on the label
transition surfaces).
%
To define a \textcolor{Christoph}{new} set of simplices, we demand that no
faces are flipped, $\forall \hat{s}\in \hat{S}, \exists s\in S$ with
$\hat{s} \cap s = \hat{s}$. Then one can find a new variable set and
data cost $\hat{\rho}$ with the same energy: %.
%
%The algorithm is simple:
\textcolor{Christoph}{ % shorter
We} initialise the new variables from the
continuous solution at the respective location, and find new
$\rho_{\hat{v}}$ by integration.
%, initialized from $(x^*, \lambda^*, \theta^*)$
%The s
\textcolor{Christoph} % shorter
{Subsequent} minimisation in the refined mesh can only decrease the
energy.
%
The argument works in both ways: Vertices that have the same solution
as their adjacent neighbors can be removed without changing the
energy.
%
For now we stick to this simple scheme, future work might explore more
sophisticated ideas, \eg along the lines of \cite{Grinspun02}.
%

%%%%%
% END, FROM HERE ON ALL COMMENTED
%%%%%

\begin{comment}

\todo{Dual graph for grid follows P1}
\todo{no connectivity information stored (adjacent)}
\todo{Corollary refinement (E ref = e coarse) proof supplementary }
energy independent of the discretisation.  Likewise, refine our
simplex discretisation at will, % and even coarsen while we can ensure
that the energy can only decrease during these operations, more
sophisticated, \eg following \cite{Grinspun02}, are postponed for
future work adaptiveness -> refine energy .. relation ..
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% need to add stuff about the model of haene !
\begin{comment}
%
To address 3D semantic segmentation and geometry reconstruction in a
joint fashion, we follow the approach of \cite{HaneZCAP13}.
%
The model employs an implicit volumetric representation, allowing for
arbitrary but closed and oriented topology of the resulting surface.
%
One limitation of that model is its huge memory consumption, which we
address with our spatially adaptive scheme, without loss in quality.

\subsection{Discrete Formulation}
%
%To that end
In \cite{HaneZCAP13} a bounding box of the region of interest is
subdivided into regular and equally sized voxels $s\in\Omega$.
%
The model then determines the likelihood that an individual voxel is
in a certain state.
%
The scene is described by a set of labeling functions
$x_s^i\in[0,1]$, which are constant per voxel element $s$.
%\in\Omega$.
%
%which we denote by indicator functions $x_s^i\in[0,1]$.
%, which we denote by indicator functions $x^i\in[0,1]$.
%constant per voxel
%of and labels each voxel $s\in\Omega$
%
%Here $s$ denotes a voxel in the volume $\mathcal{V}$,
%determined by a bounding box.
%
As indicated by the respective function $(x^i=1)$, the voxels can take
on a state (\ie a class) $i$ out of a predefined set
$\mathcal{C}=\{0 \ldots M\}$.
%
For our urban scenario we consider a voxel to either be
\emph{freespace} ($i=0$), or occupied with
\emph{building wall}, \emph{roof}, \emph{vegetation} or \emph{ground}.
Additionally we collect objects that are not explicitly modeled in an
extra \emph{clutter} state.

%%%
The data cost $\rho_s^i$ combines evidence from depthmaps and
semantic segmentation masks, and encodes the likelihood of label $i$
at a certain voxel $s$.
\subsection{Data Term}
%
\begin{figure}[tb]
\centering
%\includegraphics[width=0.6\columnwidth]{./pictures/plotA3.pdf}
%
\vspace{-0.1cm}
\caption{%Illustration of the
Contribution to the data term %$\rho_s^i$
of the ray $r$ through pixel $p$ observing class $i$ and depth $d$,
\cf\Eqs(\ref{eq:dataclass},\ref{eq:datadepth}).
}\label{fig:data}
\vspace{-0.3cm}
\end{figure}

To define the data cost for a voxel at a certain grid resolution we
again follow \cite{HaneZCAP13}.
%
%Consider a pixel $p$ in one of the images, and let its observed depth
%and semantic class be $d$ and $i$, respectively.
%
Consider a pixel $p$ in one of the images, and let $d$ denote the
pixel's observed depth. The possible semantic classes are indexed with
$i$.
%and semantic class be $d$ and $i$, respectively.
%
Now, let $r(p,\hat{d})$ be a function that maps a depth value
$\hat{d}$ to a 3D point on the ray through $p$.
%
Then the contribution of $p$ to the energy at voxel $s$ is:
\vspace{-0.01cm}
%
\begin{subequations}
\begin{align}
\rho_s^i &:= \,\,\quad \sigma^i \,\,\textrm{if} \; r(p,d+\delta) \in s \land i\neq 0 \,\text{, and} \label{eq:dataclass}
%,\; \forall i\neq 0 \,\text{, and} \label{eq:dataclass}
%\land i\neq 0 \,\text{, and} \label{eq:dataclass}
\\
\rho_s^i &:=
\!\left\{
\vspace{-0.3cm}
\begin{array}{l@{\hspace{0.15cm}}ll}
%\beta    & \textrm{if}  \; r(p,\hat{d})\in s \land d_p<\hat{d} \land |d_p-\hat{d}| < \delta \land i\neq 0
\,\beta    & \,\textrm{if}  \;\exists\, \hat{d}: r(p,\hat{d})\in s \land 0 \!<\! d-\hat{d} \!<\! \delta \land i\neq 0
\\[1mm]
\!\!\!\!-\beta   & \,\textrm{if}  \;\exists\, \hat{d}: r(p,\hat{d})\in s \land 0 \!<\! \hat{d}-d \!<\! \delta  \land i\neq 0 \label{eq:datadepth}
%-\beta   & \textrm{if}  \; r(p,\hat{d})\in s \land d_p>\hat{d} \land |d_p-\hat{d}| < \delta \land i\neq 0 \label{eq:datadepth}
\\[1mm]
%\sigma^i & \textrm{if}  \; |d_s-\hat{d}_s+\delta| < \delta \land s \in \text{ray}(p) \land i\neq 0 \\[3mm]
\,0 & \,\text{otherwise.}
\raisetag{1.5em}
\end{array}
\right.
\end{align}
%\vspace{-0.05cm}
\end{subequations}
%
The situation is depicted in \Fig\ref{fig:data}.  $\sigma^i$ denotes
the negative log-likelihoods of observing class $i$ in the pixel.  The
$\sigma^i$ are obtained from a MultiBoost classifier. Details can be
found in the supplementary material.
%
%\remark{Maros, some more detail here.}

\Eq~\eqref{eq:datadepth} is independent of the class label $i$
and only considers voxels close to the surface, as predicted by
the depth map.  Because we seek to minimise the energy
(\Eq\ref{eq:basic}), the data cost prefers freespace for voxels in
front of the observed depth.
%
The model that underlies \Eqs~(\ref{eq:dataclass},\ref{eq:datadepth})
assumes the inlier noise in the depthmaps to be exponentially
distributed and bounded by the parameter $\delta$,
\cf \cite{HaneZCAP13}.
%
%
Assuming independence of the per-pixel observations, %in different views and pixels,
the final data costs per voxel can be accumulated over all rays. %simply
%

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
%
To address 3D semantic segmentation and geometry reconstruction in a
joint fashion, we follow the approach of \cite{HaneZCAP13}.
%
The model employs an implicit volumetric representation, allowing for
arbitrary but closed and oriented topology of the resulting surface.
%
One limitation of that model is its huge memory consumption, which we
address with our spatially adaptive scheme, without loss in quality.

\subsection{Discrete Formulation}
%
%To that end
In \cite{HaneZCAP13} a bounding box of the region of interest is
subdivided into regular and equally sized voxels $s\in\Omega$.
%
The model then determines the likelihood that an individual voxel is
in a certain state.
%
The scene is described by a set of labeling functions
$x_s^i\in[0,1]$, which are constant per voxel element $s$.
%\in\Omega$.
%
%which we denote by indicator functions $x_s^i\in[0,1]$.
%, which we denote by indicator functions $x^i\in[0,1]$.
%constant per voxel
%of and labels each voxel $s\in\Omega$
%
%Here $s$ denotes a voxel in the volume $\mathcal{V}$,
%determined by a bounding box.
%
As indicated by the respective function $(x^i=1)$, the voxels can take
on a state (\ie a class) $i$ out of a predefined set
$\mathcal{C}=\{0 \ldots M\}$.
%
For our urban scenario we consider a voxel to either be
\emph{freespace} ($i=0$), or occupied with
\emph{building wall}, \emph{roof}, \emph{vegetation} or \emph{ground}.
Additionally we collect objects that are not explicitly modeled in an
extra \emph{clutter} state.
%

\end{comment}


==> justPaperArxiv/tex/methods_save.tex <==
%
The multi-labeling
problem \cite{ChambolleCP12,Strekalovskiy11,Lellmann11,ZachHP14} in
the domain $\Omega\subset \mathbb{R}^d$ is defined by finding $m$
labeling functions $x^i:\Omega \rightarrow \{0,1\}, i=1\ldots m$ as
the solution of:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:multiLabelProblem}
%\begin{split}
\inf_{x^i} \sum_{i=1}^m \int_\Omega \rho^i(z) x^i(z) \dz + J(x^i),
\quad\textrm{s.\ t. } \sum_{i=1}^{m} x^i(z)=1 \;\forall z\in\Omega,
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
where $\rho$ models the data term for a specific label at location
$z\in\Omega$ and $J$ denotes a convex regularisation functional that enforces
the spatial consistency of the labels.
%
\textcolor{Christoph}
{
One prominent example is to chose $J:= \norm{\cdot}{_2}$, known as Total Variation,
which penalizes the perimeter of the individual regions
\cite{ChambolleCP12,NieuwenhuisTC13}.
%
Note that in the the two-label case (Potts model), this relaxation is exact
after thresholding with any threshold from the open unit
interval \cite{ChambolleCP12}.
%-> generalised Potts model -- should be clear now .. it is stupid to refer to the abstract here .. ?
}
%
Although we are ultimately interested in non-metric regularisation, we
start with the continuous, anisotropic model \cite{Strekalovskiy11},
and postpone the extension to the non-metric case to Sec.~\ref{subsec:nonmetric}.
%and postpone the extension to the non-metric case,
%and a discussion of its implications to Sec.~\ref{subsec:nonmetric}.

\vspace{-0.15cm}
\subsection{Convex Relaxation}
%
The continuous model allows for an anisotropic regulariser in $J$:
label transitions can be penalised on the area of the shared surface,
as well as on the surface normal direction.
%
This is achieved with problem-specific 1-homogeneous functions that
emerge from convex sets, so called Wulff-shapes.
%instead of unit balls.
%As mentioned, we choose for $J$ the anisotropic model of \cite{Strekalovskiy11}
%and extend it later to the non-metric case, after discretisation.
%
A relaxation of $x^i(z)\in\{ 0,1\}$ to $x^i(z)\in[0,1]$ then leads to a convex
energy, which can be written as the following saddle point problem, with primal functions $x$ and dual functions $\lambda$:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:saddle}
%\begin{split}
%&
\min_{x^i} \max_{\lambda^i} \sum_i\!\!\! \int_\Omega\!\!\!\! \rho^i\!(z) x^i(z) \!\!+\!\! \langle x^i(z), \div \lambda^i(z) \rangle \dz,
%\\
%&
\;\;
\textrm{s.t. } \lambda^i(z)\!-\!\lambda^j(z) \in W^{ij}\!\!
, %\textrm{ and }
\sum_{i=1}^{m} \!x^i(z)\!\!=\!\!1 , %\raisetag{3.5\baselineskip} %\notag
x^i(z)\!\geq\!0 .
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
%where the labeling function $x^i:\Omega \rightarrow \mathbb{R}$
The constraints have to be fulfilled for all $z\in\Omega$.
In addition to the primal variables $x^i$, we have introduced the dual
vector-field $\lambda^i:\mathbb{R}^d\rightarrow \mathbb{R}^d$, whose pairwise
differences are constrained to lie in the convex sets (Wulff-shapes) $W^{ij}$.
%
By letting these shapes take an anisotropic form, one can then encode
scene structure, \eg \cite{Strekalovskiy11,HaneZCAP13}.  For our
problem we demand Neumann conditions at the boundary of $\Omega$, \ie
$\langle \lambda^i,\nu \rangle =0,\forall z\in\partial\Omega$,
because the scene will continue beyond our domain ($\nu$ is the normal
of the domain boundary $\partial \Omega$).
%
%\todo{Test functions H1 div conforming spaces weak form .. NO}

\vspace{-0.15cm}
\subsection{Finite Element Spaces}
%
Here, we can only informally introduce the basic idea of FEM and
explain its suitability for problems of the form
\eqref{eq:saddle}. We refer to textbooks
\cite{Larson2013FEM,Brezzi1991,Duran2008} for a deeper and
formal treatment.
%
%In a nutshell, FEM consists in searching a solution of a variational problem

One way to solve ~\eqref{eq:saddle} is to approximate it at
a finite number of regular grid points, using finite
differences.
%
%The fundamental difference to FEM is that in the latter case we search
%A fundamental difference to FEM is that here we search
%A fundamental difference to FEM is that here we search
\textcolor{Christoph}{FEM instead searches} %shorter !
for a solution in a finite-dimensional vector space;
this \emph{trial} space is a subspace of the space in which the exact
solution is defined.
%
To that end, one chooses a suitable basis for the \emph{trial} space,
with basis functions of finite support, as well as an
appropriate \emph{test} function space.
%These must not necessarily coincide \cite{Duran2008}. % petrov galerkin
%
FEM methods then find approximate solutions to variational problems by
identifying the element from the \emph{trial} space that is orthogonal to all
functions of the \emph{test} function space.
% orthogonal means wrt inner product, given by integral (function space inner product)
For our saddle-point problem, we can instead identify the \emph{trial} space with
our primal function space and the \emph{test} space with its dual counterpart.
% then eg. max -> neccessary condition is derivative == 0 ; which is
%
Now, we can apply the same principles, and after discretisation our
solution corresponds to the continuous solution defined
by the respective basis.
%which we will in the following. %derive from here.
%
\begin{comment}
% SHORTEN !!
%Note, that consider sequences of subspaces converging to the original space.
We do not perform any convergence analysis, which would be to
consider sequences of subspaces converging to the original space.
This topic goes beyond the scope of this work.
%
The interested reader is referred to \cite{Bartels12}
for a study \wrt Total Variation.
%
Further, we are only dealing with the convex relaxation \eqref{eq:saddle}
of the original problem \eqref{eq:multiLabelProblem}.
%
\end{comment}
% shorter !
%Because we are dealing with the convex relaxation \eqref{eq:saddle}
%of the original problem \eqref{eq:multiLabelProblem}, we are not
%analyzing the convergence properties of our method.
%
%
%but also due to the complexity
%of an analysis of convergence we
%refer the interested reader to \cite{Bartels12} for a
%study concerning Total Variation.
%
% beyond the scope of this work.
%
%We consider An analysis of the convergence of goes beyond the scope of this work.
As \eqref{eq:saddle} is already a relaxation of the original
problem \eqref{eq:multiLabelProblem}, we do not present an analysis of
convergence at this point.
%
Instead, the reader is referred to \cite{Bartels12} for an
introduction to this somewhat involved topic.
%for a study concerning Total Variation.
%

In order to choose a space with good approximation properties and
suitable basis functions, we tesselate our domain into simplices.
%To define our subspace we assume a tesselation of our domain into simplices.
%To define our subspace we tesselate of our domain into simplices.
% or in next senstence more form.. to define our subspace we let
%
More formally, we define $M\!=\!\{F,V,S\}$ to be a simplex mesh with
vertices $v\!\in\! V, v\!\in\!\mathbb{R}^d$, faces $f\!\in\! F$ defined by $d$,
%vertices
and simplices $s\!\in\! S$, defined by $d\!+\!1$ vertices that
partition $\Omega$: $\cup_k s_k=\Omega, s_l\cap s_k\!=\!f_{l,k}\!\in\! F$
-- \ie two adjacent simplices share only a single face.
%
%In this work we let
In this work, for a specific set of vertices $V$, we select M to be
the corresponding Delaunay tetrahedralisation of $\Omega$
%
and only consider explicit bases. In particular, we
focus on the Lagrangian (P1) basis, which we use in the following to
derive our framework; and on the Raviart-Thomas (RT) basis.
Details for the latter are given in the supplementary material.
%, for lack of space.
%
The main difference between them is that P1 leads to piecewise linear
solutions, which must be thresholded, while RT leads to a constant
labeling function per simplex, similar to discrete MAP solutions on CRFs.
%
We note that constant labeling can lead to artefacts, such that the
adaptiveness of the FEM model becomes even more important.

%Both derivations share similar principles:
The idea of both derivations is similar:
\emph{(i)} select a basis for our primal (P1) or dual (RT) variable set,
\emph{(ii)} find a suitable form via the divergence theorem and Fenchel duality,
\emph{(iii)} extend to the non-metric case, following a principle we term ''label mass preservation''.
%Apply To fulfill our constraint set
%a complete
%derivation similar
%
\vspace{-0.5cm}
\subsection{Lagrange Elements}
%
%The Lagrange $\textrm{P}^k(M)$ basis functions describe a
%div-conforming \textcolor{red}{the expression ``div-conforming'' is a
%bit too abstract to understand for most readers} polynomial basis of
%order $k\!+\!1$ on our simplex mesh $M$.
%
The Lagrange $\textrm{P}^k(M)$ basis functions describe a
\emph{conforming} polynomial basis of
order $k\!+\!1$ on our simplex mesh $M$, \ie its elements
belong to the Hilbert space of differentiable function with
finite Lebesgue measure on the domain $\Omega$:
$\textrm{P}^k(M)\subset H^1(\Omega):= \{ p\in L^2(\Omega),\nabla p\in(L^2(\Omega)^d) \}$.
%
%here, on a
%simplex mesh $M=\{F,V,S\}$ with vertices $v\in V, v\in\mathbb{R}^d$
%faces $f\in F$ defined by $d$ vertices and
%simplices $s\in S$, defined by $d+1$ vertices, that partition $\Omega$:
%$\cup_k s_k=\Omega, s_l\cap s_k=f_{s,k}\in F$.
%Here, two simplices share a single face.
%
We are interested in the Lagrange basis of first order, $\textrm{P}^1(M)$:
%
\vspace{-.125cm}
\begin{align}
P^1(M) \!\!:=\! \{\! p\!:\Omega\!\rightarrow\! \mathbb{R} | p \!\in\! C(\Omega), \,p(x)\!:=\!\sum_{s\in S} c_s\trans x + d_s, c_s\!\in\!\mathbb{R}^d, d_s\!\in \!\mathbb{R},
\textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else}\} .
\vspace{-.125cm}
\end{align}
%
We construct our linear basis with functions that are defined
for each vertex $v$ of a simplex $s$ and can be described in
local form with barycentric coordinates:
\vspace{-0.125cm}
\begin{equation}\label{eq:bariz}
p^{1}_{s,v}(x)   := \alpha_v\; \textrm{with } x=\sum_{v\in s} \alpha_v v, \; \sum_{v\in s} \alpha_v=1, \; \alpha_v\geq0 \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else}.
\vspace{-0.125cm}
\end{equation}
%
In each simplex, one can define a scalar field $\phi_s(x)\in\mathbb{R}$ and
compute a gradient in this basis that will be constant
per simplex $s$ (\textit{cf.} Fig. \ref{fig:lagrange_elements}):
\vspace{-0.125cm}
\begin{equation}\label{eq:gradient}
\phi_s(x) := \sum_{v\in s} \phi_v p^{1}_{s,v} \; \textrm{ and } \nabla \phi_s = \sum_{v\in s} \phi_v J_{v},
\vspace{-0.125cm}
\end{equation}
%
with coefficients $\phi_v\in \mathbb{R}$. $J_{v}\in\mathbb{R}^d$
denotes a vector that is normal to the face $f_v$ opposite node $v$,
has length $\frac{|f_v|}{|s|d}$, and points towards the simplex centre.
%
$|f_v|$ denotes the area of the face $f_v$,
and $|s|$
%$\frac{1}{d\!\cdot\!(d+1)}|s|$
the volume of the simplex $s$
(\cf \Fig\ref{fig:lagrange_elements} and supplementary material).
%

\begin{comment}
\textcolor{Christoph}{save space put in supp.:}
It is easy to see that the gradient of $\phi_t$ in (\ref{eq:gradient})
 fulfills $\langle v_l-v_k; \nabla \phi_t \rangle =
f_l-f_k$.
\Ie integration along the edge leads to the respective change
in $\phi_t$.  After collecting a sufficient number linear equations of this
form, one can directly solve the linear system.
By noting that $J_{v}$ is orthogonal to all edges that do not involve
vertex $v$ we arrive at \eqref{eq:gradient}.
\end{comment}
%

\begin{figure}[tb]
\begin{center}
   %\vspace{-3mm}
   \includegraphics[width=0.85\linewidth]{figures/lagrange_elements_v2.png}
\end{center}
   %\vspace{-6.25mm}
   \vspace{-5mm} \caption{\textcolor{Audrey}{\textit{Left:} Illustration of P1 basis function shape. \textit{Middle:} Scalar field defined as a convex combination of basis coefficients. \textit{Right:} Gradient definition in a simplex (\ref{eq:gradient}).}}
\label{fig:lagrange_elements}
\vspace{-4mm}
\end{figure}

\subsection{Discretisation}
\label{subsec:discretisation}
%
To apply our Lagrange basis to \eqref{eq:saddle} we first
make use of the divergence theorem:
%
\vspace{-0.075cm}
\begin{equation}\label{eq:p1_div}
%\begin{split}
\int_\Omega \langle x^i(z), \div \lambda^i(z) \rangle \dz =
\;
\int_\Omega \langle \nabla x^i(z), \lambda^i(z) \rangle \dz -
\underbrace{\int_{\partial\Omega} \langle \nu(z), \lambda^i(z) \rangle \dz}_{=0} .
%\end{split}
\vspace{-0.25cm}
\end{equation}
%
The latter summand vanishes by our choice of $\lambda$.
%
Our approach for a discretisation in the Lagrange basis is to
choose the labeling function $x^i\in P^1(M)$.
%The respective dual (\emph{test}) space consists of constant
%vector-field per simplex and thus also our dual vector-field
%$\lambda^i_{|s}\in\mathbb{R}^d$ is constant.
This implies that our dual space consists of constant vector-fields
per simplex: $\lambda^i_{s}\in\mathbb{R}^d$.
%
To fulfill the constraint set in \eqref{eq:saddle} we have to verify
that, per simplex, the $\lambda^i_{s}$ lie in the respective Wulff-shape.
%
%Naturally, we receive $\lambda^i_{|s}$ constant per simplex,
% similar to the gradient \eqref{}.
%Further, we observe that the constraints in \eqref{eq:saddle} are
%trivial to verify, the $\lambda^i$ are constant per simplex $s$,
%thus it is sufficient to verify that each constant vector lies in the
%respective Wulff-shape.
The simplex constraints on the $x^i$ have to be modeled per vertex.
According to \eqref{eq:bariz}, the labeling functions are convex
combinations of their values at the vertices and thus stay within the
simplex.
%
%Within the simplices the labeling functions are convex combinations
%of their values at the vertices, and thus stay inside the convex shape.

We also have to convert the continuous data costs $\rho^i$ into a
cost per vertex $\rho^i_v$, which can be achieved by
convolving the continuous cost with the respective basis function:
$\rho^i_v := \int_\Omega \sum_{s\in\mathcal{N}(v)} \phi_{s}(x) \rho^i(x)\dx$.
In practice, the integral can be computed by sampling $\rho$.
% todo also in sec 4 -> can go, save space
%
%After applying \eqref{eq:p1_div}, the energy \eqref{eq:saddle}
%in the discrete setting becomes:
%
% save a line, move above eq.: actually the shitty format uses the line to increase white space..
Integrating the right hand side in \eqref{eq:p1_div} over the simplex
$s$ leads to a weighting with its volume $|s|$ and the
energy \eqref{eq:saddle} in the discrete setting becomes:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:pd1_discrete}
%\begin{split}
\min_{x^i}\max_{\lambda^i}
\sum_v \rho^i_v x_v^i \!+\! \sum_s |s| \langle \nabla x^i, \lambda_s^i \rangle \;\; \textrm{s.t. }
%\\
(\!\lambda_s^i-\lambda_s^j\!)\! \in\! W^{ij} \;\forall i\!<\!j,\; s\in S
, %\textrm{ and }
\sum_{i=1}^{m} \!x_v^i\!\!=\!\!1, \; x_v^i\!\geq\!0 \;\forall v\!\in\! V. %\raisetag{2.5\baselineskip}
%\end{split}
\vspace{-0.1cm}
\end{equation}
%
% save a line, move above eq.:
%The weighting term $|s|$ arises from integrating the
%right hand side in \eqref{eq:p1_div} %cost of the regularizer
%over the simplex $s$.
%
%
%reflects that the cost induced by the
%regularizer has to be integrated over the simplex $s$.
%
%follows from the fact that one has to integrate over
%the volume of the simplex, similar to the suggested definition of
%$\rho^i_v$ given above.

\subsection{Non-metric extension}
\label{subsec:nonmetric}
%
To start with, we note that a non-metric model does not exist in the
continuous case \cite{maggi2012sets} and our extension works
only \emph{after} the discretisation into the FEM basis.  Please refer
to the supplementary material for an in-depth discussion.
%
\textcolor{Christoph}
{
%Note that in contrast to, for instance stereo estimation, our label
Further, we remark that our label
set consists of semantic categories without any natural order, %that do not possess
which furthermore would be required to hold even for our direction
dependent regulariser.
Consequently, we cannot order our labels such that our regulariser
forms a metric on the label set.
}
%
%This leads to the situation that we cannot find an order of our
%label set which allows our regulariser to be metric,
%\ie $\forall i<j<k: |y^{ij}|_W + |y^{jk}|_W \geq |y^{ik}|_W$.
%
%However, it was shown, \eg\cite{ZachHP14}, that a regularizer in the form
%of \eqref{eq:tranform1} transforms any non-metric cost to the metric case
%The situation is depicted in \Fig\ref{fig:xxx}.
%
%
%It should be noted that, since our model is designed for the
%non-metric relaxation of \cite{ZachHP14},
%which does not posses a continuous counterpart
%convergence to the continuous solution cannot be shown.
%
%
To allow for non-metric regularisation we transform our constraint set
($\lambda^i-\lambda^j\in W^{ij}$), by introducing auxiliary
variables $z^{ij}$ and Lagrange multipliers $y^{ij}$, and exploiting
Fenchel-Duality:
%
%We now simplify our constraint set ($\lambda^i-\lambda^j\in W^{ij}$),
%to transform our energy to utilise non-metric
%Wulff-shapes.
%
%To that end, we introduce auxilliary variables $z^{ij}$ and
%Lagrange multipliers $y^{ij}$ and exploit Fenchel-Duality:
%
\vspace{-0.1cm}
\begin{equation}\label{eq:tranform1}
%\begin{split}
\max_{\lambda_s^{i},z_s^{ij}}\min_{y_s^{ij}}
\sum_{i<j}
\langle (\lambda_s^i-\lambda_s^j)-z^{ij}, y_s^{ij} \rangle - \delta_{W^{ij}}(z_s^{ij})
=
\max_{\lambda_s^{i}}\min_{y_s^{ij}}
\sum_{i<j}
- \langle (\lambda_s^i-\lambda_s^j), y_s^{ij} \rangle + || y_s^{ij} ||_{W^{ij}}.
%\end{split}
\vspace{-0.1cm}
\end{equation}
%\sum_v \rho^i_v x_v^i + |s| || y_s^{ij} ||_{W^{ij}}
The dual functions of the indicator functions for the convex
sets $W^{ij}$ are 1-homogeneous, of the form
$|| \cdot ||_{W^{ij}} \!:=\! \sup_{w\in W^{ij}} w\trans \cdot$.
%
%After rearranging terms and ignoring data term %, regularisers
%simplex constraints
%and also the weighting term $|s|$ for now,
%
\textcolor{Christoph}
{
%As explained, there is no order of our
%label set that allows to formulate our regulariser as a metric,
%
%Recall that we cannot order our labels such that
%our regulariser forms a metric on the label set,
Recall that the metric property:
$\forall i\!<\!j\!<\!k: |y^{ij}|_{W^{ij}} + |y^{jk}|_{W^{jk}} \geq |y^{ik}|_{W^{ik}}$
does not hold for our label set.
%
It was shown, \eg\cite{ZachHP14}, that a regularizer in the form
of \eqref{eq:tranform1} transforms any non-metric cost to the metric case.
%In other words \eqref{eq:pd1_discrete} cannot handle non-metric regularisers.
For an example consider \Fig\ref{fig:non-metricness}.
Here, larger penalties for the transition between labels 0 and 2 will be
replaced by encoding both transitions from label 0 to 1 and 1 to 2 together.
%with a detour via label 1.
To prevent this, we replace the $y^{ij}$ with direction dependent variables
$x^{ij}$: % and demand the transported label mass in $x^{ij}$ to be positive.
%
%by the transition via label 1
%cost by the non-metric
%expensive transition
%After rearranging
%To that end,
We rearrange \eqref{eq:tranform1}
}
and combine the first summand % in \eqref{eq:tranform1}
with the regulariser
from \eqref{eq:pd1_discrete} to arrive at the following equations
(for now ignoring $|s|$):
%
\vspace{-0.1cm}
\begin{equation*}
\sum_s \sum_i\langle \nabla x^i, \lambda_s^i \rangle
-  \sum_i \langle \lambda_s^i, \sum_{j\neq i} \left(y_s^{ij}[i<j]-y_s^{ji}[i>j] \right)\rangle, % + || y_s^{ij} ||_{W^{ij}},
\vspace{-0.1cm}
\end{equation*}
%
with $[\cdot]$ denoting Iverson brackets.
%
Let $x^{ij}:= [y^{ij}]_+$ and $x^{ji}:= [-y^{ji}]_+$,
where $[\cdot]_+:=\max(0,\cdot)$. Expanding the gradient
\eqref{eq:gradient} we get, per  simplex $s$,
%
\vspace{-0.1cm}
\begin{equation}
\sum_i \sum_{v\in s} \lambda^i_s x_v^i( [J_{v}]_+ - [-J_{v}]_+)
- \langle \lambda_s^i, \sum_{j:i\neq j} (x^{ij}-x^{ji}) \rangle,
\vspace{-0.14cm} % todo set to 0.44 and shorter .. but looks a bit off not totally though
\end{equation}
which we analyse further to achieve non-metric costs.
%
%To arrive at the discrete non-metric form,
It was observed in \cite{ZachHP14} that the $x^{ij}\in\mathbb{R}^d$
can be interpreted as encoding the ``label mass'' that transitions
from label $i$ to label $j$ in a specific direction.
%, encoded by the variables.
%
Positivity constraints (by definition) on the $x^{ij}$ avoid
the transport of negative label mass.
%
%
%\footnote{A ``positive'' direction for each component is arbitrarily,
%but consistently defined by the coordinate system.} %
%
%Further the gradient $\nabla x^i$ has to be explained
To anchor transport of mass on the actual mass of label $i$ present at
a vertex, we introduce the variables $x^{ii}$ for the mass that
remains at label $i$, and split the above constraints into two separate sets
with the help of additional dual variables $\theta$:
%
\vspace{-0.075cm}
\begin{equation}\label{eq:nonMetric}
%
\lambda^i_s (\sum_{v\in s} x_v^i [ J_{v}]_+ - \sum_j x_s^{ij}) +
\theta^i_s  (\sum_{v\in s} x_v^i [-J_{v}]_+ - \sum_j x_s^{ji}) +
\sum_{i,j} \delta_{\geq0}(x_s^{ij}).
\vspace{-0.075cm}
\end{equation}
%

\begin{figure}[t]
\begin{center}
   %\vspace{-1mm}
   \includegraphics[width=0.9\linewidth]{figures/non-metricness_v3.png}
\end{center}
   %\vspace{-6.25mm}
%   \vspace{-5mm} \caption{\textcolor{Christoph}{\textit{Left:} Without our non-metric extension,
%	optimization \wrt \eqref{eq:pd1_discrete} can lower transition costs between labels via an
%	intermediate label (here from 0 to 2 via label 1).
%	\textit{Right:} To prevent this, we use direction dependent transition variables $x^{ij}$.
%	}}
   \vspace{-5mm} \caption{\textcolor{Christoph}{\textit{Left:} Without our non-metric extension,
	optimization \wrt \eqref{eq:pd1_discrete} can lower transition costs between labels via an
	intermediate label (here from 0 to 2 via 1).
	\textit{Right:} A solution is to split the gradients of the indicator fct. and use direction dependent transition variables $x^{ij}$. %of the $x^i$ indicator fcts.
	}}
%
%   \vspace{-5mm} \caption{\textcolor{Audrey}{\textit{Left:} Synthetic scenes illustrate the effect of using (\ref{eq:pd1_discrete}) without the non-metric extension. For a transition \textit{building} to \textit{sky}, which should be highly penalized, the paid cost is in reality smaller, \textit{ie.} like if it was a proper transition \textit{building} to \textit{roof} and \textit{roof} to \textit{sky}. This results in the apparition of several unwanted transitions \textit{building} to \textit{sky} in our reconstruction. \textit{Right:} To circumvent it, the non-metric extension should be applied in order to obtain a correct assigned cost.}}
\label{fig:non-metricness}
\vspace{-3mm}
\end{figure}
%
\noindent
Note that this construction is only possible because our
elements (simplices) are of strictly positive volume,
in contrast to zero sets in $\Omega$ \wrt the Lebesgue measure.
%
%Further notice 1-homogeneous function
%which, again, are mandatory for the continuous case.
%and ensure that
%
Finally, we can write down our discrete energy in the Lagrange basis
defined on the simplex mesh $M$:
%
\vspace{-0.001cm}
\begin{equation}\label{eq:final}
\begin{split}
\min_{x^i, x^{ij}} \max_{\lambda^i,\theta^i}
%
&
\sum_{v\in V} \sum_i \rho^i_v x_v^i + \delta_{\Delta}(x_v^i) + \sum_{i<j} \sum_{s\in S} |s| || x_s^{ij}-x_s^{ji} ||_{W^{ij}} +
\\
&
\sum_s \sum_i \theta^i_s  (\sum_{v\in s} x_v^i [-J_{v}]_+ - \sum_j x_s^{ji})
%\\
+
%&
\sum_s \sum_i \lambda^i_s (\sum_{v\in s} x_v^i [ J_{v}]_+ - \sum_j x_s^{ij}) +
\sum_{i,j} \delta_{\geq0}(x_s^{ij}), \raisetag{3.5\baselineskip}
\end{split}
\vspace{-0.075cm}
\end{equation}
%
where we have moved the weighting with $|s|$ from the constraint set
to the regulariser, and denote by $\delta_{\Delta}(\cdot)$ the
indicator function of the unit simplex.
%




\vspace{-0.075cm}
\section{Semantic Reconstruction Model}\label{subsec:implementation}
%
A prime application scenario for our FEM multi-label energy model
\eqref{eq:final} is 3D semantic reconstruction.
%with scenes dominated by larger constant regions.
%where larger regions of constant labelings.
%
%
%We focus on an urban scenario and encode with
%As indicated by the respective function $(x^i=1)$, the voxels can take
%on a state (\ie a class) $i$ out of a predefined set
%$\mathcal{C}=\{0 \ldots M\}$.
%
In particular, we focus on an urban scenario and let our labeling
functions encode \emph{freespace} ($i=1$), \emph{building wall},
\emph{roof}, \emph{vegetation} or \emph{ground}.
Objects that are not explicitly modeled are collected in an
extra \emph{clutter} class.
%
We define the data cost $\rho$ at a 3D-point $x\in\Omega$ as in
\cite{HaneZCAP13}: project
$x$ into the camera views $c\in\mathcal{C}$, and retrieve the
corresponding depth $\hat{d}_c(x)$ and class likelihoods
$\sigma_c^i(x)$ from the image space.
%
The $\sigma^i$ are obtained from a MultiBoost classifier. For the depth we
look at the difference between the actual distance $d_c(x)$ to the
camera and the observed depth: $d(x,c):=d_c(x)-\hat{d}_c(x)$.
%
For the \emph{freespace} label we always set the cost to 0, for $i\neq
1$ we define:
%
%and also the distance of $x$
%to the camera $d_c(x)$ and use to define the distance between current and observed depth value.
%Then we can assign for $i\neq0$ \rho^i(x)
\vspace{-0.075cm}
\begin{equation}\label{eq:datacost}
\rho^i(x)\!:=\!\sum_{c\in\mathcal{C}}\! \sigma_c^i(x)[(k\!-1\!)\epsilon\leq d(x,c) \leq k\epsilon] +
\beta [|d(x,c)|\leq k\epsilon] \sign(d(x,c)).
%\rho^i(x)\!:=\!\sum_{c\in\mathcal{C}}\! \sigma_c^i(x)[(k\!-1\!)\epsilon\leq d_c(x)\!-\!\hat{d}_c(x)\leq k\epsilon] +
%\beta [|d_c(x)\!-\!\hat{d}_c(x)|\leq k\epsilon] \sign(d_c(x)\!-\!\hat{d}_c(x))
\vspace{-0.075cm}
\end{equation}
% todo nice figure in supplementary !! like integration thing !
%
% space ?
%The situation is depicted in \Fig\ref{fig:data}.  $\sigma^i$ denotes
%the negative log-likelihoods of observing class $i$ in the pixel.
%Details can be found in the supplementary material.
%
This model assumes independence of the per-pixel observations, and
exponentially distributed inlier noise in the depthmaps, bounded by a
parameter $k\epsilon$ (k=3 in practice). It is essentially a
continuous version of \cite{HaneZCAP13}, see that paper for details.
%
%Assuming independence of the per-pixel observations, %in different views and pixels,
%the final data costs per voxel can be accumulated over all rays. %simply
%
%
\textcolor{Christoph}{
The parameter $\epsilon$ provides a lower bound for the minimal height
of the simplices of our tesselation and thus defines the target
resolution of our method.
%bounds the minimal height of the simplices of our tesselation from below.
}
%
The discretisation of the data cost involves a convolution with the
respective basis functions, which can be approximated via sampling.
Please refer to the supplementary material for details.
%
% too long .. ?
%
\begin{comment}
%
Although we could employ importance sampling to define the data cost
$\rho^i_v$ and thus directly couple data term computation with the
construction of $M$, we resort to a much simpler strategy.
%
In \cite{HaneZCAP13} the data cost is evaluated on a regular grid, by
reprojecting grid vertices into the images, computing the data term and
adding the respective contribution to the grid location.
%
This corresponds to integrating the data cost within the respective
Voronoi-area of a vertex: the latter is proportional to the number of
regular samples falling within a Voronoi-cell, \ie have the respective
vertex as nearest neighbour.  Summing up the individual contribution
thus directly corresponds to integrating the data term within the
Voronoi region.
%
This procedure could easily be extended to importance sampling,
but it is not the computational bottleneck of the method, so we prefer
the simpler regular strategy.%
\end{comment}
%
%
The Wulff-shapes $W^{ij}$ in \eqref{eq:final} are given as the
Minkowski sum of the $L_2$-Ball,
$B^2_{\kappa^{ij}}:=\{x\in\mathbb{R}^d| \|x\|_2 \leq \kappa^{ij}\}$
and an anisotropic shape $\Psi^{ij}$:
$W^{ij}:= \Psi^{ij} \oplus B^2_{\kappa^{ij}}$.
%
In the isotropic part, $\kappa^{ij}$ contains the neighbourhood statistics
of the classes. The anisotropic part $\Psi^{ij}$ models the likelihood
of a transition between classes $i$ and $j$ in a certain direction.
\textcolor{Christoph}{
\Fig\ref{fig:wulff_shape} (a,b) provides an example.
}
%
\textcolor{Christoph}{
For our 3D reconstruction we prefer flat, horizontal structures in the model
for the following label transitions:
ground-freespace, ground-building, building-roof, ground-vegetation
and roof-freespace.
%
We utilize a second prior that prefers vertical boundaries at the transitions
between building-freespace and building-vegetation.
More details on the exact form of the shapes can be found in \cite{HaneZCAP13}.
}
%

\begin{figure}[tb]
\begin{center}
   \vspace{-1mm}
   \includegraphics[width=0.9\linewidth]{figures/wulffshape_finitediff_split.png}
\end{center}
   %\vspace{-6.25mm}
   \vspace{-5mm}
%	\caption{\textcolor{Audrey}{Not sure about this figure....}}
\caption[Optional caption for list of figures]{
\textcolor{Christoph}{
 \emph{(a):} Wulff-shape (\emph{red}) with isolines.
 \emph{(b):} Minkowski sum of two Wulff-shapes.
 \emph{(c):} Simplices are split after inserting new vertices (blue) close to the surface (green).
	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
\emph{(d):} Finite differences on a regular grid
  (\cite{HaneZCAP13}) only cover constraints in \emph{green} areas,
	the P1 basis covers all of the domain $\Omega$.
	}
}
\label{fig:wulff_shape}
\vspace{-3.5mm}
\end{figure}




The energy \eqref{eq:final} is already in primal-dual form, such that
we can apply the minimisation scheme of \cite{chambolle11}, with
pre-conditioning \cite{Pock11}.
%
That numerical scheme requires us to project onto shapes that are
Minkowski sums of convex sets.  In our case, the sets are simple and
the projection onto each shape can be performed in closed form.
%
We employ a Dykstra-like projection scheme \cite{Dykstra}, which
avoids storing additional variables and proves remarkably efficient,
see supplementary material.
%
We also project the labeling functions $x^i$ directly onto the unit
simplex \cite{WangC13a}.
%
In order to extract the transition surface, we employ a variant of marching
tetrahedra (triangles) \cite{treece1999mtet}, using the isolevel at $0.5$
for each label.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\subsection{Comparison to Voxel Based Tesselation}

%\mypargraph{Remarks. }
% $x^i_{\hat{v}}:=\sum_{v\in s}  \alpha_v(\hat{v} )x^i_{v}$
%

%
% Other VERSION
%
%\begin{figure}[ht]
%\centering
%\subfigure[]{
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%    \label{fig:grid}
%}
%\hspace{0.4cm}
%\subfigure[]{
%\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%    \label{fig:refine}
%}
%
%\caption[Optional caption for list of figures]{(a) \emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%  \emph{Right:} Gradient definition in a simplex (\eqref{eq:gradient}).
% (b)\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface (green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%}
%\label{fig:subfigureExample}
%\end{figure}


%\begin{figure}[tb]
%\begin{minipage}{.575\textwidth}
%  \centering
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%	\vspace{-0.2cm}
%  \caption{\emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%%\emph{Right:} Gradient definition in a simplex \eqref{eq:gradient}.
%	}\label{fig:grid}
%\end{minipage}
%%
%\hspace{0.175cm}
%\begin{minipage}{.4\textwidth}
%  \centering
%	\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%		\vspace{-0.2cm}
%  \caption
%	{\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface (green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%	}\label{fig:refine}
%	%
%\end{minipage}
%\vspace{-4mm}
%\end{figure}



%\begin{figure}[tb]
%%\centering
%\begin{minipage}{.575\textwidth}
%  \centering
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
%\includegraphics[height=1.5cm,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual_brighter.pdf}
%\includegraphics[height=1.6cm]{./figures/subdiv_Grad1.pdf}
%%	\vspace{-0.4cm}
%  \caption{\emph{Left:} Finite differences on a regular grid
%  (\emph{left}, \cite{HaneZCAP13}) only cover constraints
%  in \emph{green} areas, the P1 basis covers all of the domain
%  $\Omega$.
%\emph{Right:} Gradient definition in a simplex (\eqref{eq:gradient}).
%	}\label{fig:grid}
%\end{minipage}
%%
%\hspace{0.175cm}
%\begin{minipage}{.4\textwidth}
%  \centering
%	\includegraphics[height=1.5cm,trim={7cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%		%\vspace{-0.4cm}
%  \caption
%	{\emph{Left:} Simplices are split after inserting new vertices (blue) close to the surface %(green).
%	\emph{Right:} Initialization of vertices after refinement. % via barycentric coordinates.
%	}\label{fig:refine}
%	%
%\end{minipage}
%\vspace{-5mm}
%\end{figure}


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[tb]
\centering
\includegraphics[width=0.175\columnwidth,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_primal.pdf}
\includegraphics[width=0.175\columnwidth,trim={5cm 1cm 1cm 0 },clip]{./figures/subdiv_dual.pdf}
\includegraphics[width=0.15\columnwidth]{./figures/subdiv_Grad.pdf}
\hspace{0.3cm}
\includegraphics[width=0.375\columnwidth,trim={5cm 0cm 0cm 0 },clip]{./figures/subdiv_x2.pdf}
%
\vspace{-0.1cm}
\caption{%Illustration of the
.
}\label{fig:grid}
\vspace{-0.3cm}
\end{figure}
\end{comment}
%
We conclude with two interesting remarks.
%
First, note that a tesselation with a regular grid \cite{HaneZCAP13} can be
seen as a simplified version of our discretisation in the $P^1$ Lagrange basis.
% consider the special case of a regular grid
%Consider a vertex set aligned on a grid, then we can a special case of
In \Fig \ref{fig:wulff_shape}(d) %\ref{fig:grid},
we consider the 2D case of the regular grid
%interpretation
used in \cite{HaneZCAP13}. Here, variables are defined at voxel level.
%
In its dual graph, the vertex set consists of the corners of the primal
grid cubes, leading to shifted indicator variables.  %are thus shifted;
Per vertex the data term is mainly influenced from the cost in its Voronoi area.
%
%and the dual cells correspond to the Voronoi cells of the
%dual vertex set.
%
Similarly, \cite{HaneZCAP13} evaluates the data cost at grid centers,
approximately corresponding to integration within the
respective Voronoi-area of grid cell. %a dual vertex.
%
Furthermore, taking finite differences in this regular case
corresponds to verifying constraints for %computing the gradient and
only one of the two triangles (\Fig\ref{fig:wulff_shape}(d)). %(\Fig \ref{fig:grid}).
The supplementary material includes a more formal analysis.
%
\begin{comment}
In the following we will show that a tesselation on a regular grid
\cite{HaneZCAP13} is a special case of our discretisation in the $P^1$ Lagrange
basis.
%
To that end, we consider the dual graph of a regular grid, \ie a grid where the
vertex set consists of corners of the primal grid cubes, and dual cells
correspond to voronoi cells \wrt new set of dual vertices.
%
For our regular grid the dual mesh simply becomes a shifted regular
grid \ref{fig:wulff_shape}(c). %\ref{fig:dual}.
%
\end{comment}

Second, our formulation is adaptive, in the sense
of \cite{BlahaVRWPS16}: Hierarchical refinement of the tesselation can
only decrease our energy. Hence, our scheme is applicable when refining
the model on-the-fly.
%
We again must defer a formal proof to the supplementary material and
give an intuitive, visual explanation in \Fig\ref{fig:wulff_shape}(c). % \Fig\ref{fig:refine}.
%
%Assume that we found an optimal solution $(x^*, \lambda^*, \theta^*)$
\textcolor{Christoph}{Assume that  $(x^*, \lambda^*, \theta^*)$ is an optimal solution}
for a certain triplet $M=\{F,V,S\}$.  Then a refined tesselation
$\hat{M}=\{\hat{F},\hat{V},\hat{S}\}$ can be found by introducing
additional vertices, \ie $V\subset\hat{V}$ (ideally on the label
transition surfaces).
%
To define a \textcolor{Christoph}{new} set of simplices, we demand that no
faces are flipped, $\forall \hat{s}\in \hat{S}, \exists s\in S$ with
$\hat{s} \cap s = \hat{s}$. Then one can find a new variable set and
data cost $\hat{\rho}$ with the same energy: %.
%
%The algorithm is simple:
\textcolor{Christoph}{ % shorter
We} initialise the new variables from the
continuous solution at the respective location, and find new
$\rho_{\hat{v}}$ by integration.
%, initialized from $(x^*, \lambda^*, \theta^*)$
%The s
\textcolor{Christoph} % shorter
{Subsequent} minimisation in the refined mesh can only decrease the
energy.
%
The argument works in both ways: Vertices that have the same solution
as their adjacent neighbors can be removed without changing the
energy.
%
For now we stick to this simple scheme, future work might explore more
sophisticated ideas, \eg along the lines of \cite{Grinspun02}.
%

%%%%%
% END, FROM HERE ON ALL COMMENTED
%%%%%

\begin{comment}

\todo{Dual graph for grid follows P1}
\todo{no connectivity information stored (adjacent)}
\todo{Corollary refinement (E ref = e coarse) proof supplementary }
energy independent of the discretisation.  Likewise, refine our
simplex discretisation at will, % and even coarsen while we can ensure
that the energy can only decrease during these operations, more
sophisticated, \eg following \cite{Grinspun02}, are postponed for
future work adaptiveness -> refine energy .. relation ..
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% need to add stuff about the model of haene !
\begin{comment}
%
To address 3D semantic segmentation and geometry reconstruction in a
joint fashion, we follow the approach of \cite{HaneZCAP13}.
%
The model employs an implicit volumetric representation, allowing for
arbitrary but closed and oriented topology of the resulting surface.
%
One limitation of that model is its huge memory consumption, which we
address with our spatially adaptive scheme, without loss in quality.

\subsection{Discrete Formulation}
%
%To that end
In \cite{HaneZCAP13} a bounding box of the region of interest is
subdivided into regular and equally sized voxels $s\in\Omega$.
%
The model then determines the likelihood that an individual voxel is
in a certain state.
%
The scene is described by a set of labeling functions
$x_s^i\in[0,1]$, which are constant per voxel element $s$.
%\in\Omega$.
%
%which we denote by indicator functions $x_s^i\in[0,1]$.
%, which we denote by indicator functions $x^i\in[0,1]$.
%constant per voxel
%of and labels each voxel $s\in\Omega$
%
%Here $s$ denotes a voxel in the volume $\mathcal{V}$,
%determined by a bounding box.
%
As indicated by the respective function $(x^i=1)$, the voxels can take
on a state (\ie a class) $i$ out of a predefined set
$\mathcal{C}=\{0 \ldots M\}$.
%
For our urban scenario we consider a voxel to either be
\emph{freespace} ($i=0$), or occupied with
\emph{building wall}, \emph{roof}, \emph{vegetation} or \emph{ground}.
Additionally we collect objects that are not explicitly modeled in an
extra \emph{clutter} state.

%%%
The data cost $\rho_s^i$ combines evidence from depthmaps and
semantic segmentation masks, and encodes the likelihood of label $i$
at a certain voxel $s$.
\subsection{Data Term}
%
\begin{figure}[tb]
\centering
%\includegraphics[width=0.6\columnwidth]{./pictures/plotA3.pdf}
%
\vspace{-0.1cm}
\caption{%Illustration of the
Contribution to the data term %$\rho_s^i$
of the ray $r$ through pixel $p$ observing class $i$ and depth $d$,
\cf\Eqs(\ref{eq:dataclass},\ref{eq:datadepth}).
}\label{fig:data}
\vspace{-0.3cm}
\end{figure}

To define the data cost for a voxel at a certain grid resolution we
again follow \cite{HaneZCAP13}.
%
%Consider a pixel $p$ in one of the images, and let its observed depth
%and semantic class be $d$ and $i$, respectively.
%
Consider a pixel $p$ in one of the images, and let $d$ denote the
pixel's observed depth. The possible semantic classes are indexed with
$i$.
%and semantic class be $d$ and $i$, respectively.
%
Now, let $r(p,\hat{d})$ be a function that maps a depth value
$\hat{d}$ to a 3D point on the ray through $p$.
%
Then the contribution of $p$ to the energy at voxel $s$ is:
\vspace{-0.01cm}
%
\begin{subequations}
\begin{align}
\rho_s^i &:= \,\,\quad \sigma^i \,\,\textrm{if} \; r(p,d+\delta) \in s \land i\neq 0 \,\text{, and} \label{eq:dataclass}
%,\; \forall i\neq 0 \,\text{, and} \label{eq:dataclass}
%\land i\neq 0 \,\text{, and} \label{eq:dataclass}
\\
\rho_s^i &:=
\!\left\{
\vspace{-0.3cm}
\begin{array}{l@{\hspace{0.15cm}}ll}
%\beta    & \textrm{if}  \; r(p,\hat{d})\in s \land d_p<\hat{d} \land |d_p-\hat{d}| < \delta \land i\neq 0
\,\beta    & \,\textrm{if}  \;\exists\, \hat{d}: r(p,\hat{d})\in s \land 0 \!<\! d-\hat{d} \!<\! \delta \land i\neq 0
\\[1mm]
\!\!\!\!-\beta   & \,\textrm{if}  \;\exists\, \hat{d}: r(p,\hat{d})\in s \land 0 \!<\! \hat{d}-d \!<\! \delta  \land i\neq 0 \label{eq:datadepth}
%-\beta   & \textrm{if}  \; r(p,\hat{d})\in s \land d_p>\hat{d} \land |d_p-\hat{d}| < \delta \land i\neq 0 \label{eq:datadepth}
\\[1mm]
%\sigma^i & \textrm{if}  \; |d_s-\hat{d}_s+\delta| < \delta \land s \in \text{ray}(p) \land i\neq 0 \\[3mm]
\,0 & \,\text{otherwise.}
\raisetag{1.5em}
\end{array}
\right.
\end{align}
%\vspace{-0.05cm}
\end{subequations}
%
The situation is depicted in \Fig\ref{fig:data}.  $\sigma^i$ denotes
the negative log-likelihoods of observing class $i$ in the pixel.  The
$\sigma^i$ are obtained from a MultiBoost classifier. Details can be
found in the supplementary material.
%
%\remark{Maros, some more detail here.}

\Eq~\eqref{eq:datadepth} is independent of the class label $i$
and only considers voxels close to the surface, as predicted by
the depth map.  Because we seek to minimise the energy
(\Eq\ref{eq:basic}), the data cost prefers freespace for voxels in
front of the observed depth.
%
The model that underlies \Eqs~(\ref{eq:dataclass},\ref{eq:datadepth})
assumes the inlier noise in the depthmaps to be exponentially
distributed and bounded by the parameter $\delta$,
\cf \cite{HaneZCAP13}.
%
%
Assuming independence of the per-pixel observations, %in different views and pixels,
the final data costs per voxel can be accumulated over all rays. %simply
%

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{comment}
%
To address 3D semantic segmentation and geometry reconstruction in a
joint fashion, we follow the approach of \cite{HaneZCAP13}.
%
The model employs an implicit volumetric representation, allowing for
arbitrary but closed and oriented topology of the resulting surface.
%
One limitation of that model is its huge memory consumption, which we
address with our spatially adaptive scheme, without loss in quality.

\subsection{Discrete Formulation}
%
%To that end
In \cite{HaneZCAP13} a bounding box of the region of interest is
subdivided into regular and equally sized voxels $s\in\Omega$.
%
The model then determines the likelihood that an individual voxel is
in a certain state.
%
The scene is described by a set of labeling functions
$x_s^i\in[0,1]$, which are constant per voxel element $s$.
%\in\Omega$.
%
%which we denote by indicator functions $x_s^i\in[0,1]$.
%, which we denote by indicator functions $x^i\in[0,1]$.
%constant per voxel
%of and labels each voxel $s\in\Omega$
%
%Here $s$ denotes a voxel in the volume $\mathcal{V}$,
%determined by a bounding box.
%
As indicated by the respective function $(x^i=1)$, the voxels can take
on a state (\ie a class) $i$ out of a predefined set
$\mathcal{C}=\{0 \ldots M\}$.
%
For our urban scenario we consider a voxel to either be
\emph{freespace} ($i=0$), or occupied with
\emph{building wall}, \emph{roof}, \emph{vegetation} or \emph{ground}.
Additionally we collect objects that are not explicitly modeled in an
extra \emph{clutter} state.
%

\end{comment}


==> justPaperArxiv/tex/related_savety.tex <==
\textcolor{Konrad}{Related is too long, and contains irrelevent stuff that we needed to cite only for the CVPR octree paper.}

\vspace{1em}

\textcolor{Konrad}{So far, literature on FEM entirely missing. Say in which fields FEM is popular or has been developped for mathematically similar problems. And cite something, at least textbooks or review articles.}

\vspace{1em}

\textcolor{Konrad}{The following -- conceptual hacks in Zach and Strekalowsky -- should be mentioned explicitly. Of course be polite, don't attack them and maybe mention that in practice it might still work well enough. But let the reader know that, as part of our contribution, we rectify/solidify theoretically some existing work that has not been thought through in as much detail by earlier authors.}
Zach: not constant per element == voxel interpretation by haene not correct (not mention explicitly)
it is P1 function per element so linear per voxel
Strekalowsky non-metric not continuous : impossible (do not state this explicitly)
finite elements for TV \cite{Bartels12}
\cite{reddy2005introduction}
\cite{Ritz1909}

Large-scale 3D city reconstruction is an important application of
computer
vision, \eg \cite{Gallup2010,lafarge_pami13,kuschk-et-al-iccv2013}.
%
Research aiming at purely geometric surface reconstruction rarely uses
volumetric representations, though, because of the high demands \wrt
memory and computational resources.
%
In this context \cite{lafarge_ijcv12} already used a preceding
semantic labeling to improve geometry reconstruction, but not vice
versa.

Initial attempts to jointly perform geometric and semantic
reconstruction started with depth maps \cite{Ladicky10}, but later
research, which aimed for truly 3-dimensional reconstruction from
multiple views, switched to a volumetric representation
\cite{HaneZCAP13,Bao13,Kundu14,Savinov15,vineet2015icra}, or in rare cases meshes \cite{Cabezas15}.
%
The common theme of these works is to allow interaction between 3D
depth estimates and appearance-based labeling information, via class
specific shape priors. Loosely speaking, the idea is to obtain at the
same time a reconstruction with locally varying, class-specific
regularization; and a semantic segmentation in 3D, which is then
trivially consistent across all images.
%
The model of \cite{HaneZCAP13} employs a discrete, tight, convex
relaxation of the standard multi-label Markov random field
problem \cite{ZachHP14} in 3D, at the cost of high memory
consumption and computation time.
%
Here, we use a similar energy and optimization scheme, but
significantly reduce the run-time and memory consumption, while
retaining the advantages of a joint model.
%
\cite{Kundu14} also jointly solve for class label and occupancy state,
but model the data term with heuristically shortened ray potentials
\cite{LiuC10,Savinov15}.
%
Yet, the representation inherits the asymptotic dependency
on the number of pixels in the input images.
%
\cite{Kundu14} also resort to an octree data structure to save memory,
which is fixed in the beginning according to the ray
potentials, contrary to our work, where it is adaptively refined.
% KONRAD - following not true here. If anything, our work is a
% ``principled combination of\cite{Labatut07} and \cite{haene13}.
%
% This is perhaps also the work that comes closest to ours in terms of
% large-scale urban modeling, but (like other semantic reconstruction
% research) it uses only street-level imagery, and thus only needs to
% cover the vicinity of the road network, whereas we reconstruct the
% complete scene.

Since the seminal work \cite{Curless1996} volumetric reconstruction
has evolved remarkably.
%
% ALL COVERED LATER, NO NEED TO REPEAT
%\cite{Kazhdan:2006:PSR,Zach2007_Range,Labatut07,VogiatzisETC07,Bolitho:2007:MSO,Furu:2010:PMVS,LiuC10,Cremers-Kolev-pami11,Jancosek11,kbc-pami11,HaneZCAP13,KostrikovHL14}.
%
%Most of them have in common that they
Most methods compute a distance field or indicator function in the
volumetric domain, either from images or by directly merging
several 2.5D range scans.
%
Once that representation has been established, the surface can be
extracted as its zero level set, \eg
\cite{Lorensen1987,Kazhdan2007}.
%
%general indicator or distance function
%TV-Fusion \cite{Zach2007_Range}
%the level-set of an implicit 3D function is a fundamental
%technique for many computer graphics applications.

Many volumetric techniques work with a regular partitioning of the
volume of
interest \cite{Zach2007_Range,zach2008fast,LiuC10,Cremers-Kolev-pami11,kbc-pami11,KostrikovHL14,Savinov15}. % Kazhdan:2006:PSR,
%
%The first three methods \cite{Kazhdan:2006:PSR,Zach2007_Range,zach2008fast} are variational -- yawn who cares
% NOTE SURE THE FOLLOWING IS NEEDED
The data term per voxel is usually some sort of signed distance
generated from stereo
maps, \eg \cite{Zach2007_Range,zach2008fast}. Beyond stereo
depth, \cite{Cremers-Kolev-pami11} propose to also exploit silhouette
constraints as additional cue about occupied and empty space.

\textcolor{Konrad}{following paragraph too long! shorten/remove as fr as possible}
Going one step further, \cite{LiuC10,Savinov15} model, for each pixel
in each image, the visibility along the full ray. Such a geometrically
faithful model of visibility, however, leads to higher-order
potentials per pixel, comprising all voxels intersected by the
corresponding ray.
%
Consequently the memory consumption is no longer proportional to the
number of voxels, but depends on the number of ray-voxel
intersections, which can be problematic for larger image sets and/or
high-resolution images.
%
In contrast, the memory footprint of our method (and of others that
include visibility locally \cite{Zach2007_Range,HaneZCAP13}) is linear
in the number of voxels, and thus can be reduced efficiently by
adaptive discretization.

%Octree used for xx
%non batch method:
%depth sensor data
%Octree: \cite{Steinbruecker-etal-iccv13} ours is smarter with shared pointers - well depends on the application actually so not true.
%Octree: \cite{Steinbruecker-etal-icra14} octree for data fusion, adopts the approach of \cite{Curless1996}.
%incremental meshing - thus the distance function is updated over time; at the detail level/scale of the octree cell determined by the distance to the sensor.
%% mesh by marching cubes
%We similarly employ an octree data structure which is incrementally adapted, yet
%also adaptive : \cite{Sinha07}

\textcolor{Konrad}{Following shold be more prominent. Like Haene is, from the outsider's view an extension of voxel occupancy labeling to multiple labels; ours is, in the same way, an extension of tetrahedron occupany labeling to multiple labels}
\cite{Labatut07,vu12} deviate from a regular partitioning of the volume,
and instead start from a Delauney tetrahedralization of a 3D point
cloud (from multi-view stereo). The tetrahedrons are then labeled % by
the optimization of a discrete energy, as being either as empty or
occupied, and the final surface is composed of triangles that are
shared by tetrahedrons with different labels.
%
The idea was extended by \cite{Jancosek11}, who focus on
visibility to also recover weakly supported objects.

\textcolor{Konrad}{Whole following paragraph too long! Needed at all?}
In fact even the well-known PMVS multi-view stereo
method \cite{Furu:2010:PMVS} originally includes volumetric surface
reconstruction from the estimated 3D points and normals.
%
To that end, the Poisson reconstruction method \cite{Kazhdan:2006:PSR}
was adopted, which aligns the surface with a guidance
vector field (given by the estimated normals).
%which computes the indicator function of the scene
%(inside or outside of the 3D model) by exploiting that its gradient
%is zero almost everywhere, except at points on the surface.
%
%whose underlying sparse least squares system minimizes the difference of the
%gradient of the indicator function to a sparsely sampled guidance vector
%field, given by the previously reconstructed normals at the patch %which is given
%centers.
%
%That reconstruction method was later extended by \cite{Bolitho:2007:MSO} to
%an adaptive octree representation, which, in combination with a
%cascadic multigrid solver, \eg \cite{Briggs2000,Grinspun02}, leads to
%a significant speed-up.
%
%\novel{ %adaptive
%Taking advantage of the octree representation of \cite{Kazhdan:2006:PSR},
%a later extension \cite{Bolitho:2007:MSO} could further utilize a
%cascadic multigrid solver, \eg \cite{Briggs2000,Grinspun02},
%leading to a significant speed-up.
The octree representation of \cite{Kazhdan:2006:PSR}, was later combined
\cite{Bolitho:2007:MSO} with a cascadic multigrid solver,
\eg \cite{Briggs2000,Grinspun02}, leading to a significant speed-up.
%}
%
The framework is eminently suit\-able for large scale processing, but
the least-squares nature inherited from the original Poisson
formulation makes it susceptible to outliers.
%
In contrast, our formulation can use robust error functions to handle
noisy input. The price to pay is a more involved optimization problem
instead of a simple linear system.
%
We furthermore exploit that high precision is only needed at voxels
close to the surface;
%
representing large regions, that have a constant semantic label, with
many voxels appears wasteful.
%
A similar idea was utilized by \cite{Agarwala07} in the context of
stitching images in the gradient domain.
%
%\novel{
%%% I HAD TO SQUEEZE IT -- so please double check:
Contrary to prior work \cite{Kazhdan:2006:PSR,Bolitho:2007:MSO,ssd11},
our octree structure is not predetermined by the input data,
%fixed in advance
%according to the input data, % access to probabilities not MAP
%but adapted based on the current solution,
but refined adaptively,
%based on a coarse solution which approximates the final reconstruction.
such that we can exploit the per-class probabilities %(transition)
rather than only a minimal energy solution.
%Here, we exploit having access to actual probability values instead
%of only a minimal energy solution.
%Here, we exploit that explicit probabilities deliver more information
%than a minimal energy solution.
% (\cf \Sec\ref{sec:}).
%
%Compared to refining all voxels with data, we experience no loss of
%performance and avoid many unnecessary splits that would otherwise
%be evoked by our noisy depth maps.
Compared to refining all voxels with data, we can avoid many
unnecessary splits that would otherwise be invoked by noise in the
depth maps.
%
%In our experience
%}
%
%\begin{comment}

% KONRAD - following not true, we do no multigrid or adaptive here
%
%One can interpret our method as a combination of multi-grid
%(coarse-to-fine) reconstruction on a volumetric
%pyramid \cite{Zach2007_Range,zach2008fast}, and adaptive hierarchical
%refinement, \eg \cite{HornungK06}.
%, where also a preliminary
%reconstruction at a coarser discretization serves to decide where to
%refine the grid.
%
%We also refine selectively, and initialize the solver
%from previous results for faster convergence.


==> justPaperArxiv/tex/suppContinuous.tex <==
%
\subsection{Non-Metricness: Continuous vs. Discrete}
%
\begin{comment}
Although we finally desire an extension to \emph{non-metric} priors $J$ that
are of major importance for the success for our application scenario, we cannot
achieve this directly and have to go for a small detour.
\Ie the model has to be extended \emph{after} the discretisation into the
finite elementy (FEM) basis.
\end{comment}

We briefly explain why a non-metric model does not exist in the continuous
case without additional constraints on the functions spaces. % if we require lower semi-continuity of our energy \cite{maggi2012sets}.
%
Without additional constraints, one can always introduce a zero set, 
assigned to a label $j$, between any two
regions labeled $i$ and $k$, \ie a set with a Lebesque measure of $0$ in the
domain space.
Consequently the potentially higher transition cost for a non-metric label pair
$i,k$ compared to the sum of costs between $i,j$ and $j,k$
can always be avoided in the limit and non-metric energies are underestimated.
%implicitly becomes a metric.
%
%\todo{need some continuous equations here}.
%
%In practice, this is can become a serious problem, because the energy of the
%computed solution will be underestimated.
%in general by measuring the perimeter
%optimisation scheme will underestimate the energy of the computed solution.
%and the assigned energy will  not match.
%
In other words, let $S$ be a segmentation of $\Omega$ into regions $S^i$ and $S^k$,
labeled with $i$ and $k$ respectively, with costs that do not fulfill the triangle
inequality \wrt another label $j$.
Then one can find a sequence of segmentations $S^n:=\{S_i^n, S_j^n, S_k^n\}$
with $\displaystyle S=\lim_{n\to\infty} S^n$, \ie the label $j$ disappears in the limit case,
such that $\displaystyle \lim_{n\to\infty}\inf E(S^n) < E(S)$.
Hence, the metric property is a necessary condition for the lower
semi-continuity of our energy functional.
%On the other hand every metric regulariser implies the lsc. of our energy functional.
%
%
\begin{comment}
%labeled with $i,j,k$ respectively, such
% with non-metric transition costs, \ie the transition cost between
%$i,k$ does not fulfill the triangle inequality
%compared to $i,j$ and $j,k$
%is penalised
%
%that assign a higher penalty
%to label transitions $i,k$ compared to the sum of penalties between
%$i,j$ and $j,k$,
%one can find
we can find a sequence of segmentations
$S^n:=\{S_i^n, S_j^n, S_k^n\}$ with $S=\lim_{n\to\infty} S^n$
%
labeled with $i,j,k$ respectively, such
that $S_j^n$ disappears in the limit $n\rightarrow\infty$
for which $\displaystyle \lim_{n\to\infty}\inf E(S^n) < E(S)$.
%
%such that converges to the wrong solution
%triangle ineq implies lsc
\end{comment}
%
Methods that try to avoid this problem,
\eg by demanding Lipshitz continuity of the labeling functions
%and thus to guarantee convergence for non-metric priors
are an active research area,
\eg \cite{BreMas15}, but go beyond the scope of this work.

Any discretization of our domain will ultimately consist of only a finite number of 
elements of measurable ($>0$) volume. 
Thus, the label $j$ in the example above does not disappear %in the solution 
and the computed energy matches the solution. 
%
\begin{comment}
In the discrete setting, we have committed ourselves to a certain
tesselation of our domain and % we cannot find such a sequence;
the area assigned to a certain label cannot become a zero set. 
Thus the label $j$ does not disappear in the solution.
The computed energy matches the solution.
\end{comment}
%
%if one demands that each assignment
%\ie will the label will finally occur in the solution.
%
%However, this shows that our discrete solution will not converge to the
%continuous solution in the non-metric setting,
%
Our analysis implies, however, that a discrete solution in the non-metric
setting does not have a continuous counterpart and any investigation of the
limit case, \ie convergence analysis, 
after infinite refinements of the tesselation, is unreasonable. 
%
%It should be noted that, since our model is designed for the 
%non-metric relaxation of \cite{ZachHP14},  
%which does not posses a continuous counterpart 
%convergence to the continuous solution cannot be shown. 
%
%
%any convergence analysis to the continuous solution
%of our discrete energy is unreasonable.
%in the limit,
%our discrete solution will also converge to the wrong solution

%However, to perform infinite refinement steps appears unpractical and further more unreasonable

%  of the level of refinement of the tesselation of the domain.
%Thus, we start from the less general model of \cite{Strekalovskiy11}.

\subsubsection{Gradient in the Lagrange basis}
%
We repeat the statement from the paper, namely that 
we can compute a gradient in the P1 (Lagrange) basis that is 
constant per simplex $s$ and given by:
%
\begin{equation}\label{eq:gradient}
\nabla \phi_s = \sum_{v\in s} \phi_v J_{v}.
\end{equation}
%
Here, the coefficients $\phi_v\in \mathbb{R}$ and 
$J_{v}\in\mathbb{R}^d$ denote a vector, normal to the face $f_v$,
opposite to the node $v$ pointing inwards,
towards the center of the simplex with length $\frac{|f_v|}{|s|}$.
%
recall that $|f_v|$ denoted the area of the face $f_v$
and $|s|$ the volume of the simplex $s$ (\cf supplementary).

At first notice that the gradient of $\phi_t$ in (\ref{eq:gradient})
has to fulfill $\langle v_l-v_k; \nabla \phi_t \rangle = \phi_l-\phi_k$.
\Ie integration along the edge leads to the respective change
in $\phi_t$.  After collecting a sufficient number linear equations of this
form, one can directly solve the linear system. 
By noting that $J_{v}$ is orthogonal to all edges that do not involve 
vertex $v$ we arrive at \eqref{eq:gradient}.


\subsection{Data Term for Lagrange basis} % version of our
%
Although we could employ importance sampling to define the data cost 
$\rho^i_v$ and thus directly couple data term computation with the 
construction of $M$, we resort to a much simpler strategy. 
%
In \cite{HaneZCAP13} the data cost is evaluated on a regular grid, by
reprojecting grid vertices into the images, computing the data term and
adding the respective contribution to the grid location.
%
This corresponds to integrating the data cost within the respective
Voronoi-area of a vertex: the latter is proportional to the number of
regular samples falling within a Voronoi-cell, \ie have the respective
vertex as nearest neighbour.  Summing up the individual contribution
thus directly corresponds to integrating the data term within the
Voronoi region.
%
This procedure could easily be extended to importance sampling,
but it is not the computational bottleneck of the method, so we prefer
the simpler regular strategy.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Raviart-Thomas Elements}
%
The Raviart-Thomas $\textrm{RT}^k(M)$ basis functions describe a
div-conforming polynomial basis of order $k\!+\!1$, here, on a
simplex mesh $M=\{F,V,S\}$ with vertices $v\in V, v\in\mathbb{R}^d$
faces $f\in F$ defined by $d$ vertices and
simplices $s\in S$, defined by $d+1$ vertices, that partition $\Omega$:
$\cup_k s_k=\Omega, s_l\cap s_k=f_{s,k}\in F$.
Here, two simplices share a single face.
%
\begin{align*}
&
RT^0(M) := \{ p:\Omega\rightarrow \mathbb{R}^d | p(x):=\sum_{s\in S} p_s(x) \textrm{ with }
\\ &
p_s(x):=c_s x + d_s, c_s\!\in\!\mathbb{R}, d_s\!\in \!\mathbb{R}^d,
\textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else},
\\
&
\textrm{and } p_s(x) \textrm{ is continuous for } x\in f_v(s) \textrm{ in direction } \nu_{f_v}
\}.
%
\end{align*}
%
Here we used $\nu_{f_v}$ to denote the normal of face $f_v$ of simplex s,
which, by convention, is located opposite to the vertex $v$.
%

We construct our linear basis with functions that are defined % \ie $k=0$
for each face $f_v$ opposite to a vertex $v$ in a simplex $s$
and can described in a local form as follows:
\begin{equation*}
p^{0}_{l,s,v}(x) := (x-v) |f_v|/|s| \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else},
\end{equation*}
where we let $|f_v|$ denote the area of the face and $|s|$ $d$ times
the volume of the simplex.
We can read of $\textrm{div}(p^{0}_{s,v})=|f_v|/|s|$.
Let $\nu_{f_v}$ be the normal of face $f_v$, then the basis functions
fulfill
%
\begin{equation}\label{eq:property_RT}
\langle p^{0}_{s,u}(x), \nu_{f_v} \rangle := [u=v] \;\forall x\in f_v,
\end{equation}
where we make use of the Iverson bracket $[\cdot]$.
%
These basis functions make up the global function space by enforcing a
consistent orientation, for example we can distinguish for each face $f$
two simplices $s^+$ and $s^-$ analysing the scalar product of
the vector $\mathbf{1}$ and the normal $\nu^\pm_f$ of the shared face $f$
pointing outwards into each simplex.
Wlog we define $s^\pm$ via %the sign of
$\sign \langle \nu^\pm_f; \mathbf{1}\rangle$.
%s^\pm:= and $s^-$ accordingly.
The global basis functions per face $f_v$ opposite to
vertex $v$ are then given by:
\begin{equation}\label{eq:RT_global_basis}
p^{0}_{s^\pm,v} := \pm (x-v) |f_v|/|s^\pm| \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else}.
\end{equation}
%
In each simplex a vector-field $\phi_s(x)\in\mathbb{R}^d$ is defined in
the following manner (with coefficients $\phi_v\in \mathbb{R}$):
\begin{equation*}
\phi_s(x) := \sum_{v\in s} \phi_v p^{0}_{s,v}.
\end{equation*}
%
By construction (\cf \eqref{eq:RT_global_basis}, \eqref{eq:property_RT}),
the vector-field has to be continuous along the face $x\in f_v$
normal direction $\nu_{f_v}$, \ie for neighbouring faces $\forall\phi_{s^\pm}$
we have: %s^\pm$
%orthogonal to the face
%
\begin{equation}\label{eq:RT-edgeSKP}
\langle \phi_{s^\pm}(x), \nu_{f_v} \rangle = \pm \langle x-v_\pm,\nu_{f_v}\rangle |f_v|/|s^\pm| \phi_{f_{v^\pm}} = \phi_{f_{v^\pm}}.
\end{equation}
%
Thus, our function is $\phi$ is a RT function iff for all neighbouring $s\pm$
faces we have $\phi_{f_{v^+}}=\phi_{f_{v^-}}$, or in other words basis
coefficients only exist for faces of the simplices.

Furthermore, the variables we are interested in are the labeling
functions $x^i$,
%
%which will be the dual multipliers of our objective in
%\eqref{eq:E-dual} after replacing the '$\min$' by its fenchel conjugate
%again
%(leading to the re-introduction of the indicator functions $x^i$
%and simplex constraints for these).
%The solution will be constant per simplex, \ie a piecewise constant labeling.
%Given a tesselation $S$ of $\Omega$, our
which are members of our test function space composed
of piecewise constant functions per simplex:
\begin{align*}
U^0(M):= \{ u:\Omega\rightarrow \mathbb{R} | &u(x):=\sum_{s\in S} u_s(x), \textrm{ with }
\\ &
u_s(x)=u_s \textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else}\}.
\end{align*}
%
With this choice, the defined basis is div-conforming:
%, the equivalence to the continuous case can be shown with the help of the divergence theorem:
%
\begin{align}\label{eq:discDiv}
& %_{|S}
\int_\Omega u(x) \div{}\phi(x) \dx = \sum_{s\in S}\int_S u_s \div\phi(x) \dx %\nonumber
=
\\
&
\sum_{s\in S}\int_{\partial S} \!\!\!\!u_s \langle \phi(x), \nu \rangle \dz
%\\
=
\sum_{\overset{v\in s}{s\in S}} u_s \phi_v |f_v|
=
\sum_{s\in S} u_s \div\phi(x) |s|.\nonumber
\end{align}
%p^{0}_{s,v}
Again, $\nu$ encodes the face normal $f_v$ of simplex $s$ pointing outwards.

Before we can utilise our new basis to discretise \eqref{eq:saddle} we need
proof that it is sufficient to enforce the constraints on our dual functions
$\phi$ in \eqref{eq:saddle} at the vertices of the simplex $s$.
%face midpoints $x_{f_v}$
to ensure the constraints are also valid for any point in the whole simplex.
%
The Wulff shapes are convex as are the linear inequalities in \eqref{eq:E-dual},
thus it is sufficient to proof that the vector field $\phi(x)$ at any
point $x\in s$ can be written as a convex combination:
%
\begin{equation*}%\label{eq:convexComb_edgemid}
\phi(z) = \sum_{f_v\in s} \alpha_{z,f_v} \phi(v), \textrm{with} \sum_{f_v\in s} \alpha_{z,f_v}=1.
\end{equation*}
%
After some algebra, it turns out that if $x=\alpha_i v_i$ then %$\phi(x) = (1-d\alpha_i) \phi(x_{f_{v_i}})$
$\alpha_{x,f_v}:=(1-d\cdot\alpha_i)$ encode this convex combination.

The same is true if the functions are evaluated at the vertex positions:
\begin{equation}\label{eq:convexComb}
\phi(x) = \sum_{v\in s} \alpha_{v} \phi(v), \textrm{with} \sum_{v\in s} \alpha_v=1.
\end{equation}
%
This has the additional advantage that one face in the summation can be
ignored and evaluation at a point can be written as a matrix
multiplication with an invertible matrix
(from relevant basis coefficients to value at the point and back).
This is useful in the linear constraint set.

In a simplex $s$ the RT function $\phi_s(x) := \sum_{v\in s} \phi_v p^{0}_{s,v}(x)$
evaluated at the face midpoint $x_{f_v}=1/d\sum_{w \in s, w\neq v}w$ becomes:
\begin{equation*}
\phi_s(x_{f_v}) = - \phi_v\frac{|f_v|}{|s|} v -\!\!\!\!\! \sum_{w\in s, w\neq v} \!\!\!\!\!\frac{w}{d}(\phi_w\frac{|f_w|}{|s|} -\!\!\!\! \sum_{u\in s, u\neq w}\!\!\! \phi_u\frac{|f_u|}{|s|}).
\end{equation*}

If we utilise the values at the vertices we receive a seemingly simpler but
certainly more compact representation. To compute $\phi(v)$ for some vertex $v$
of the simplex $s$, we can compose a linear map:
\begin{align}\label{eq:project_matrix}
  \phi(v) = \sum_{v_i\in s, v_i\neq v} (v-v_i) \frac{|f_{v_i}|}{|s|} \phi_{v_i},
\end{align}
%
which can also be assembled in matrix form $\phi_s(v) = M_{s,v} \phi_{s,v}$,
with an invertible matrix $M_{s,v}$.
The columns are a weighted combination of the edges towards the
vertex $v$ to be evaluated \eqref{eq:project_matrix}.
Apparently we can compute all but one coefficient from the value at one
vertex already.
%


\begin{comment}
\begin{comment}
% too complex for now.

\subsection{Raviart-Thomas Elements}
%
The Raviart-Thomas $\textrm{RT}^k(M)$ basis functions describe a
div-conforming polynomial basis of order $k\!+\!1$, here, on a
simplex mesh $M=\{F,V,S\}$ with vertices $v\in V, v\in\mathbb{R}^d$
faces $f\in F$ defined by $d$ vertices and
simplices $s\in S$, defined by $d+1$ vertices, that partition $\Omega$:
$\cup_k s_k=\Omega, s_l\cap s_k=f_{s,k}\in F$.
Here, two simplices share a single face.
%
\begin{align*}
&
RT^0(M) := \{ p:\Omega\rightarrow \mathbb{R}^d | p(x):=\sum_{s\in S} p_s(x) \textrm{ with }
\\ &
p_s(x):=c_s x + d_s, c_s\!\in\!\mathbb{R}, d_s\!\in \!\mathbb{R}^d,
\textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else},
\\
&
\textrm{and } p_s(x) \textrm{ is continuous for } x\in f_v(s) \textrm{ in direction } \nu_{f_v}
\}.
%
\end{align*}
%
Here we used $\nu_{f_v}$ to denote the normal of face $f_v$ of simplex s,
which, by convention, is located opposite to the vertex $v$.
%

We construct our linear basis with functions that are defined % \ie $k=0$
for each face $f_v$ opposite to a vertex $v$ in a simplex $s$
and can described in a local form as follows:
\begin{equation*}
p^{0}_{l,s,v}(x) := (x-v) |f_v|/|s| \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else},
\end{equation*}
where we let $|f_v|$ denote the area of the face and $|s|$ $d$ times
the volume of the simplex.
We can read of $\textrm{div}(p^{0}_{s,v})=|f_v|/|s|$.
Let $\nu_{f_v}$ be the normal of face $f_v$, then the basis functions
fulfill
%
\begin{equation}\label{eq:property_RT}
\langle p^{0}_{s,u}(x), \nu_{f_v} \rangle := [u=v] \;\forall x\in f_v,
\end{equation}
where we make use of the Iverson bracket $[\cdot]$.
%
These basis functions make up the global function space by enforcing a
consistent orientation, for example we can distinguish for each face $f$
two simplices $s^+$ and $s^-$ analysing the scalar product of
the vector $\mathbf{1}$ and the normal $\nu^\pm_f$ of the shared face $f$
pointing outwards into each simplex.
Wlog we define $s^\pm$ via %the sign of
$\sign \langle \nu^\pm_f; \mathbf{1}\rangle$.
%s^\pm:= and $s^-$ accordingly.
The global basis functions per face $f_v$ opposite to
vertex $v$ are then given by:
\begin{equation}\label{eq:RT_global_basis}
p^{0}_{s^\pm,v} := \pm (x-v) |f_v|/|s^\pm| \quad \textrm{if}\; x\in s \;\textrm{and}\; 0 \;\textrm{else}.
\end{equation}
%
In each simplex a vector-field $\phi_s(x)\in\mathbb{R}^d$ is defined in
the following manner (with coefficients $\phi_v\in \mathbb{R}$):
\begin{equation*}
\phi_s(x) := \sum_{v\in s} \phi_v p^{0}_{s,v}.
\end{equation*}
%
By construction (\cf \eqref{eq:RT_global_basis}, \eqref{eq:property_RT}),
the vector-field has to be continuous along the face $x\in f_v$
normal direction $\nu_{f_v}$, \ie for neighbouring faces $\forall\phi_{s^\pm}$
we have: %s^\pm$
%orthogonal to the face
%
\begin{equation}\label{eq:RT-edgeSKP}
\langle \phi_{s^\pm}(x), \nu_{f_v} \rangle = \pm \langle x-v_\pm,\nu_{f_v}\rangle |f_v|/|s^\pm| \phi_{f_{v^\pm}} = \phi_{f_{v^\pm}}.
\end{equation}
%
Thus, our function is $\phi$ is a RT function iff for all neighbouring $s\pm$
faces we have $\phi_{f_{v^+}}=\phi_{f_{v^-}}$, or in other words basis
coefficients only exist for faces of the simplices.

Furthermore, the variables we are interested in are the labeling
functions $x^i$,
%
%which will be the dual multipliers of our objective in
%\eqref{eq:E-dual} after replacing the '$\min$' by its fenchel conjugate
%again
%(leading to the re-introduction of the indicator functions $x^i$
%and simplex constraints for these).
%The solution will be constant per simplex, \ie a piecewise constant labeling.
%Given a tesselation $S$ of $\Omega$, our
which are members of our test function space composed
of piecewise constant functions per simplex:
\begin{align*}
U^0(M):= \{ u:\Omega\rightarrow \mathbb{R} | &u(x):=\sum_{s\in S} u_s(x), \textrm{ with }
\\ &
u_s(x)=u_s \textrm{ if } x\!\in\! s \textrm{ and } 0 \textrm{ else}\}.
\end{align*}
%
With this choice, the defined basis is div-conforming:
%, the equivalence to the continuous case can be shown with the help of the divergence theorem:
%
\begin{align}\label{eq:discDiv}
& %_{|S}
\int_\Omega u(x) \div{}\phi(x) \dx = \sum_{s\in S}\int_S u_s \div\phi(x) \dx %\nonumber
=
\\
&
\sum_{s\in S}\int_{\partial S} \!\!\!\!u_s \langle \phi(x), \nu \rangle \dz
%\\
=
\sum_{\overset{v\in s}{s\in S}} u_s \phi_v |f_v|
=
\sum_{s\in S} u_s \div\phi(x) |s|.\nonumber
\end{align}
%p^{0}_{s,v}
Again, $\nu$ encodes the face normal $f_v$ of simplex $s$ pointing outwards.

Before we can utilise our new basis to discretise \eqref{eq:saddle} we need
proof that it is sufficient to enforce the constraints on our dual functions
$\phi$ in \eqref{eq:saddle} at the vertices of the simplex $s$.
%face midpoints $x_{f_v}$
to ensure the constraints are also valid for any point in the whole simplex.
%
The Wulff shapes are convex as are the linear inequalities in \eqref{eq:E-dual},
thus it is sufficient to proof that the vector field $\phi(x)$ at any
point $x\in s$ can be written as a convex combination:
%
\begin{equation*}%\label{eq:convexComb_edgemid}
\phi(z) = \sum_{f_v\in s} \alpha_{z,f_v} \phi(v), \textrm{with} \sum_{f_v\in s} \alpha_{z,f_v}=1.
\end{equation*}
%
After some algebra, it turns out that if $x=\alpha_i v_i$ then %$\phi(x) = (1-d\alpha_i) \phi(x_{f_{v_i}})$
$\alpha_{x,f_v}:=(1-d\cdot\alpha_i)$ encode this convex combination.

The same is true if the functions are evaluated at the vertex positions:
\begin{equation}\label{eq:convexComb}
\phi(x) = \sum_{v\in s} \alpha_{v} \phi(v), \textrm{with} \sum_{v\in s} \alpha_v=1.
\end{equation}
%
This has the additional advantage that one face in the summation can be
ignored and evaluation at a point can be written as a matrix
multiplication with an invertible matrix
(from relevant basis coefficients to value at the point and back).
This is useful in the linear constraint set.

In a simplex $s$ the RT function $\phi_s(x) := \sum_{v\in s} \phi_v p^{0}_{s,v}(x)$
evaluated at the face midpoint $x_{f_v}=1/d\sum_{w \in s, w\neq v}w$ becomes:
\begin{equation*}
\phi_s(x_{f_v}) = - \phi_v\frac{|f_v|}{|s|} v -\!\!\!\!\! \sum_{w\in s, w\neq v} \!\!\!\!\!\frac{w}{d}(\phi_w\frac{|f_w|}{|s|} -\!\!\!\! \sum_{u\in s, u\neq w}\!\!\! \phi_u\frac{|f_u|}{|s|}).
\end{equation*}

If we utilise the values at the vertices we receive a seemingly simpler but
certainly more compact representation. To compute $\phi(v)$ for some vertex $v$
of the simplex $s$, we can compose a linear map:
\begin{align}\label{eq:project_matrix}
  \phi(v) = \sum_{v_i\in s, v_i\neq v} (v-v_i) \frac{|f_{v_i}|}{|s|} \phi_{v_i},
\end{align}
%
which can also be assembled in matrix form $\phi_s(v) = M_{s,v} \phi_{s,v}$,
with an invertible matrix $M_{s,v}$.
The columns are a weighted combination of the edges towards the
vertex $v$ to be evaluated \eqref{eq:project_matrix}.
Apparently we can compute all but one coefficient from the value at one
vertex already.
%
%
Instead of repeating the complete derivation for the P1 basis of piecewise
linear functions on our simplex partition we follow an alternative route,
which allows for additional insights into the original grid based formulation
of \cite{HaneZCAP13,ZachHP14} and is pleasantly visual.

Dual graph for grid follows P1

\end{comment}

==> justSuppArxiv/tabulars/verification.tex <==
\begin{table}[h]

  \centering
  \setlength\tabcolsep{5pt}
  %\small
  \begin{tabular}{ l|c|c|c|c|c }

Data set & Error measure & Tetra P1 & Tetra RT & Octree & MB \\ \hline
\multirow{2}{*}{Scene 1} 
 & Overall acc. [\%] & 84.0 & 81.9 & 83.9 & 82.5 \\
 & Average acc. [\%] & 81.1 & 79.1 & 80.6 & 81.4 \\

  \end{tabular}
\vspace{2mm}
\caption{Quantitative comparison of our two proposed FEM methods with octree model \cite{BlahaVRWPS16} and MultiBoost input data \cite{benbouzid_jml12}.}
\label{tab:verified}
\vspace{-0.45cm}
\end{table}


==> justSuppArxiv/tex/proofs.tex <==
\input{suppContinuous}
\begin{comment}
\subsection{Adaptiveness}\label{sec:gradient_lagrange}

\textcolor{Audrey}{TODO: Introduction of new vertices doesn't change the energy. Energy cannot increase, only decrease so energy cannot increase with introduction of new vertices. Vice versa with merging of vertices with same value.}



\subsection{Grid vs. P1}
\label{sec:grid_p1}


\subsection{Adaptiveness}
\label{sec:adaptiveness}


\subsection{Dykstra-like projection scheme}
\label{sec:optimization}

\textcolor{Audrey}{TODO: Like in the same spirit of octree supplementary.}


\subsection{Finite differences on a regular grid}
\label{sec:data_cost}

\textcolor{Audrey}{TODO: Demonstration + Figure like in our Deekit.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}


==> justSuppArxiv/tex/proofsc.tex <==
\subsection{Gradient in Lagrange basis}\label{sec:gradient_lagrange}
short proof as in why is it like this. have already





\subsection{Continuous vs Discrete}
\label{sec:continuous_discrete_discussion}







\subsection{optimization - dykstra}
\label{sec:data_cost}



\subsection{grid vs fem}
\label{sec:GridvsFEM}


\subsection{Adaptiveness}
\label{sec:adaptiveness}


\subsection{Data cost integration}
\label{sec:data_cost}



